Stationarity preserving nodal Finite Element methods for multi-dimensional linear hyperbolic balance laws via a Global Flux quadrature formulation

We consider linear, hyperbolic systems of balance laws in several space dimensions. They possess non-trivial steady states, which result from the equilibrium between derivatives of the unknowns in different directions, and the sources. Standard numerical methods fail to account for this equilibrium, and include stabilization that destroys it. This manifests itself in a diffusion of states that are supposed to remain stationary. We derive new stabilized high-order Finite Element methods based on a Global Flux quadrature: we reformulate the entire spatial operator as a mixed derivative of a single quantity, referred to as global flux. All spatial derivatives and the sources are thus treated simultaneously, and our methods are stationarity preserving. Additionally, when this formulation is combined with interpolation on Gauss-Lobatto nodes, the new methods are super-convergent at steady state. Formal consistency estimates, and strategies to construct well-prepared initial data are provided. The numerical results confirm the theoretical predictions, and show the tremendous benefits of the new formulation.

==> figures/LinAc2D_SG/errors_SUPG_GF_ord2.tex <==
20& 5.62e-03 & 5.93e-03 & 3.15e-03 & 0.00 & 0.00 & 0.00 \\ 
40& 1.37e-03 & 1.43e-03 & 7.12e-04 & 2.03 & 2.05 & 2.15 \\ 
80& 3.28e-04 & 3.41e-04 & 1.66e-04 & 2.07 & 2.07 & 2.10 \\ 
160& 7.87e-05 & 8.16e-05 & 4.01e-05 & 2.06 & 2.06 & 2.05 \\ 
320& 1.90e-05 & 1.97e-05 & 9.86e-06 & 2.05 & 2.05 & 2.03 

==> figures/LinAc2D_SG/errors_SUPG_GF_ord3.tex <==
10& 6.18e-05 & 4.62e-05 & 2.10e-05 & 0.00 & 0.00 & 0.00 \\ 
20& 4.42e-06 & 3.02e-06 & 1.41e-06 & 3.81 & 3.94 & 3.90 \\ 
40& 2.97e-07 & 1.95e-07 & 9.42e-08 & 3.90 & 3.95 & 3.90 \\ 
80& 1.92e-08 & 1.24e-08 & 6.18e-09 & 3.95 & 3.98 & 3.93 \\ 
160& 1.22e-09 & 7.81e-10 & 3.98e-10 & 3.98 & 3.99 & 3.96 

==> figures/LinAc2D_SG/errors_SUPG_GF_ord4.tex <==
6& 1.21e-05 & 8.29e-06 & 3.68e-06 & 0.00 & 0.00 & 0.00 \\ 
13& 2.67e-07 & 1.74e-07 & 6.02e-08 & 4.94 & 5.00 & 5.32 \\ 
26& 8.28e-09 & 5.32e-09 & 1.27e-09 & 5.01 & 5.03 & 5.57 \\ 
53& 2.33e-10 & 1.49e-10 & 2.04e-11 & 5.01 & 5.02 & 5.80 \\ 
106& 7.20e-12 & 4.57e-12 & 4.27e-13 & 5.02 & 5.02 & 5.58 

==> figures/LinAc2D_SG/errors_SUPG_GF_ord5.tex <==
5& 8.22e-07 & 4.37e-07 & 2.28e-07 & 0.00 & 0.00 & 0.00 \\ 
10& 1.37e-08 & 6.95e-09 & 3.14e-09 & 5.91 & 5.98 & 6.18 \\ 
20& 2.17e-10 & 1.08e-10 & 3.48e-11 & 5.98 & 6.01 & 6.50 \\ 
40& 3.38e-12 & 1.67e-12 & 3.47e-13 & 6.01 & 6.02 & 6.65 \\ 
80& 7.65e-14 & 5.76e-14 & 3.08e-15 & 5.46 & 4.86 & 6.82 

==> figures/LinAc2D_SG/errors_SUPG_GF_ord6.tex <==
4& 8.65e-08 & 4.78e-08 & 1.99e-08 & 0.00 & 0.00 & 0.00 \\ 
8& 7.10e-10 & 3.55e-10 & 1.57e-10 & 6.93 & 7.07 & 6.99 \\ 
16& 5.59e-12 & 2.65e-12 & 9.74e-13 & 6.99 & 7.07 & 7.33 \\ 
32& 5.52e-14 & 3.91e-14 & 6.50e-15 & 6.66 & 6.08 & 7.23 \\ 
64& 6.41e-14 & 6.33e-14 & 3.29e-15 & -0.22 & -0.69 & 0.98 

==> figures/LinAc2D_SG/errors_SUPG_GF_ord7.tex <==
3& 2.23e-08 & 1.00e-08 & 5.59e-09 & 0.00 & 0.00 & 0.00 \\ 
6& 9.67e-11 & 3.90e-11 & 1.95e-11 & 7.85 & 8.00 & 8.17 \\ 
13& 2.05e-13 & 8.04e-14 & 3.17e-14 & 7.96 & 8.00 & 8.30 \\ 
26& 2.57e-14 & 2.78e-14 & 2.18e-15 & 3.00 & 1.53 & 3.86 \\ 
53& 4.72e-14 & 5.02e-14 & 6.60e-15 & -0.85 & -0.83 & -1.56 

==> figures/LinAc2D_SG/errors_SUPG_ord2.tex <==
20& 8.51e-03 & 8.99e-03 & 5.49e-03 & 0.00 & 0.00 & 0.00 \\ 
40& 2.21e-03 & 2.32e-03 & 1.32e-03 & 1.94 & 1.95 & 2.06 \\ 
80& 5.63e-04 & 5.89e-04 & 3.20e-04 & 1.98 & 1.98 & 2.04 \\ 
160& 1.42e-04 & 1.48e-04 & 7.90e-05 & 1.99 & 1.99 & 2.02 \\ 
320& 3.56e-05 & 3.71e-05 & 1.96e-05 & 1.99 & 2.00 & 2.01 

==> figures/LinAc2D_SG/errors_SUPG_ord3.tex <==
10& 4.88e-03 & 5.07e-03 & 3.05e-03 & 0.00 & 0.00 & 0.00 \\ 
20& 8.76e-04 & 9.00e-04 & 5.89e-04 & 2.48 & 2.49 & 2.37 \\ 
40& 1.38e-04 & 1.41e-04 & 9.73e-05 & 2.67 & 2.67 & 2.60 \\ 
80& 1.97e-05 & 2.01e-05 & 1.43e-05 & 2.80 & 2.82 & 2.77 \\ 
160& 2.69e-06 & 2.68e-06 & 1.95e-06 & 2.87 & 2.90 & 2.87 

==> figures/LinAc2D_SG/errors_SUPG_ord4.tex <==
6& 3.01e-04 & 3.26e-04 & 1.84e-04 & 0.00 & 0.00 & 0.00 \\ 
13& 1.64e-05 & 1.55e-05 & 9.02e-06 & 3.76 & 3.94 & 3.90 \\ 
26& 1.10e-06 & 9.70e-07 & 5.69e-07 & 3.90 & 4.00 & 3.99 \\ 
53& 6.59e-08 & 5.59e-08 & 3.36e-08 & 3.95 & 4.01 & 3.97 \\ 
106& 4.17e-09 & 3.46e-09 & 2.10e-09 & 3.98 & 4.01 & 4.00 

==> figures/LinAc2D_SG/errors_SUPG_ord5.tex <==
5& 2.34e-05 & 3.13e-05 & 1.46e-05 & 0.00 & 0.00 & 0.00 \\ 
10& 1.04e-06 & 1.28e-06 & 6.23e-07 & 4.49 & 4.61 & 4.55 \\ 
20& 3.98e-08 & 4.63e-08 & 2.31e-08 & 4.71 & 4.79 & 4.76 \\ 
40& 1.40e-09 & 1.57e-09 & 7.89e-10 & 4.83 & 4.88 & 4.87 \\ 
80& 4.72e-11 & 5.10e-11 & 2.58e-11 & 4.89 & 4.94 & 4.93 

==> figures/LinAc2D_SG/errors_SUPG_ord6.tex <==
4& 1.88e-06 & 2.98e-06 & 1.31e-06 & 0.00 & 0.00 & 0.00 \\ 
8& 3.49e-08 & 5.01e-08 & 2.39e-08 & 5.75 & 5.90 & 5.77 \\ 
16& 6.06e-10 & 8.08e-10 & 4.02e-10 & 5.85 & 5.95 & 5.89 \\ 
32& 9.97e-12 & 1.27e-11 & 6.51e-12 & 5.92 & 5.99 & 5.95 \\ 
64& 1.55e-13 & 2.15e-13 & 1.04e-13 & 6.01 & 5.89 & 5.97 

==> figures/LinAc2D_SG/errors_SUPG_ord7.tex <==
3& 5.88e-07 & 8.28e-07 & 4.16e-07 & 0.00 & 0.00 & 0.00 \\ 
6& 6.90e-09 & 9.04e-09 & 4.84e-09 & 6.41 & 6.52 & 6.43 \\ 
13& 3.88e-11 & 4.93e-11 & 2.75e-11 & 6.70 & 6.74 & 6.69 \\ 
26& 3.36e-13 & 4.31e-13 & 2.41e-13 & 6.85 & 6.84 & 6.83 \\ 
53& 1.67e-14 & 1.68e-14 & 5.11e-15 & 4.22 & 4.56 & 5.41 

==> figures/LinAc2D_coriolis_vortex/big_table_ord2.tex <==
20 & 7.9e-03 & 3.9e-03 & 0.0 & 0.0 & 2.5e-03 & 1.7e-03 & 0.0 & 0.0 & 6.0e-03 & 4.7e-03 & 0.0 & 0.0 & 2.6e-03 & 2.0e-03 & 3.1 & 2.3 \\
40 & 1.6e-03 & 8.6e-04 & 2.3 & 2.2 & 6.4e-04 & 4.2e-04 & 2.0 & 2.0 & 1.3e-03 & 9.0e-04 & 2.2 & 2.4 & 6.5e-04 & 4.5e-04 & 2.0 & 2.2 \\
80 & 3.4e-04 & 1.8e-04 & 2.2 & 2.3 & 1.6e-04 & 8.9e-05 & 2.0 & 2.2 & 3.2e-04 & 1.8e-04 & 2.1 & 2.3 & 1.6e-04 & 9.1e-05 & 2.0 & 2.3 \\
160 & 8.0e-05 & 4.2e-05 & 2.1 & 2.1 & 3.9e-05 & 2.1e-05 & 2.0 & 2.1 & 7.8e-05 & 4.2e-05 & 2.0 & 2.1 & 3.9e-05 & 2.1e-05 & 2.0 & 2.1 \\
320 & 2.0e-05 & 1.1e-05 & 2.0 & 2.0 & 9.8e-06 & 5.3e-06 & 2.0 & 2.0 & 2.0e-05 & 1.0e-05 & 2.0 & 2.0 & 9.8e-06 & 5.3e-06 & 2.0 & 2.0 

==> figures/LinAc2D_coriolis_vortex/big_table_ord3.tex <==
10 & 1.1e-02 & 3.1e-03 & 0.0 & 0.0 & 7.6e-04 & 2.5e-04 & 0.0 & 0.0 & 9.0e-03 & 5.7e-03 & 0.0 & 0.0 & 8.2e-04 & 5.6e-04 & 4.3 & 4.5 \\
20 & 2.9e-03 & 4.9e-04 & 2.0 & 2.7 & 1.3e-04 & 5.1e-05 & 2.5 & 2.3 & 2.2e-03 & 1.2e-03 & 2.1 & 2.2 & 1.4e-04 & 9.0e-05 & 2.5 & 2.6 \\
40 & 7.8e-04 & 1.3e-04 & 1.9 & 1.9 & 8.2e-06 & 3.2e-06 & 4.0 & 4.0 & 6.2e-04 & 2.5e-04 & 1.8 & 2.3 & 8.7e-06 & 4.7e-06 & 4.0 & 4.3 \\
80 & 1.7e-04 & 2.9e-05 & 2.2 & 2.2 & 5.1e-07 & 2.0e-07 & 4.0 & 4.0 & 1.8e-04 & 4.1e-05 & 1.8 & 2.6 & 5.3e-07 & 2.2e-07 & 4.0 & 4.4 \\
160 & 3.2e-05 & 5.2e-06 & 2.4 & 2.5 & 3.1e-08 & 1.2e-08 & 4.0 & 4.0 & 4.8e-05 & 8.8e-06 & 1.9 & 2.2 & 3.2e-08 & 1.3e-08 & 4.0 & 4.1 

==> figures/LinAc2D_coriolis_vortex/big_table_ord4.tex <==
6 & 1.1e-02 & 2.2e-03 & 0.0 & 0.0 & 1.4e-03 & 2.2e-04 & 0.0 & 0.0 & 1.4e-02 & 1.0e-02 & 0.0 & 0.0 & 1.4e-03 & 2.8e-04 & 0.2 & 2.0 \\
13 & 1.6e-03 & 2.7e-04 & 2.5 & 2.7 & 4.6e-05 & 1.9e-05 & 4.4 & 3.2 & 2.5e-03 & 1.7e-03 & 2.2 & 2.3 & 4.7e-05 & 2.0e-05 & 4.4 & 3.4 \\
26 & 8.3e-05 & 1.2e-05 & 4.3 & 4.5 & 2.0e-06 & 4.1e-07 & 4.6 & 5.5 & 3.8e-05 & 6.7e-06 & 6.0 & 8.0 & 2.0e-06 & 4.5e-07 & 4.6 & 5.5 \\
53 & 4.3e-06 & 6.0e-07 & 4.2 & 4.2 & 5.6e-08 & 4.3e-09 & 5.0 & 6.4 & 1.8e-06 & 2.3e-07 & 4.3 & 4.7 & 5.6e-08 & 4.9e-09 & 5.0 & 6.3 \\
106 & 2.6e-07 & 3.6e-08 & 4.0 & 4.0 & 1.7e-09 & 7.9e-11 & 5.0 & 5.7 & 1.0e-07 & 1.1e-08 & 4.1 & 4.5 & 1.7e-09 & 8.8e-11 & 5.0 & 5.8 

==> figures/LinAc2D_coriolis_vortex/big_table_ord5.tex <==
5 & 2.0e-03 & 5.8e-04 & 0.0 & 0.0 & 1.6e-03 & 4.9e-04 & 0.0 & 0.0 & 2.8e-03 & 1.3e-03 & 0.0 & 0.0 & 1.6e-03 & 5.4e-04 & 2.9 & 2.6 \\
10 & 5.4e-04 & 7.6e-05 & 1.9 & 2.9 & 9.5e-06 & 2.4e-06 & 7.4 & 7.7 & 2.9e-04 & 7.0e-05 & 3.3 & 4.2 & 9.5e-06 & 2.4e-06 & 7.4 & 7.8 \\
20 & 2.3e-05 & 2.9e-06 & 4.6 & 4.7 & 4.2e-07 & 1.0e-07 & 4.5 & 4.5 & 1.4e-05 & 4.3e-06 & 4.3 & 4.0 & 4.2e-07 & 1.0e-07 & 4.5 & 4.5 \\
40 & 1.2e-06 & 1.4e-07 & 4.3 & 4.4 & 6.6e-09 & 9.5e-10 & 6.0 & 6.7 & 1.2e-06 & 1.9e-07 & 3.6 & 4.5 & 6.6e-09 & 1.1e-09 & 6.0 & 6.6 \\
80 & 4.9e-08 & 5.5e-09 & 4.6 & 4.6 & 1.1e-10 & 1.2e-11 & 6.0 & 6.4 & 8.6e-08 & 3.8e-08 & 3.7 & 2.3 & 1.1e-10 & 1.3e-11 & 6.0 & 6.4 

==> figures/LinAc2D_coriolis_vortex/big_table_ord6.tex <==
4 & 5.1e-03 & 6.5e-04 & 0.0 & 0.0 & 9.2e-04 & 2.7e-04 & 0.0 & 0.0 & 6.1e-03 & 3.0e-03 & 0.0 & 0.0 & 9.2e-04 & 3.2e-04 & 2.8 & 3.1 \\
8 & 2.0e-04 & 2.3e-05 & 4.6 & 4.8 & 1.2e-05 & 3.1e-06 & 6.3 & 6.4 & 3.0e-04 & 1.6e-04 & 4.3 & 4.3 & 1.2e-05 & 3.4e-06 & 6.3 & 6.5 \\
16 & 6.2e-06 & 6.2e-07 & 5.1 & 5.2 & 1.2e-07 & 1.8e-08 & 6.6 & 7.4 & 6.4e-06 & 1.6e-06 & 5.6 & 6.6 & 1.2e-07 & 2.2e-08 & 6.6 & 7.3 \\
32 & 1.1e-07 & 1.2e-08 & 5.8 & 5.7 & 9.0e-10 & 1.6e-10 & 7.1 & 6.8 & 5.8e-08 & 1.5e-08 & 6.8 & 6.8 & 9.1e-10 & 1.6e-10 & 7.1 & 7.1 \\
64 & 1.7e-09 & 2.0e-10 & 6.0 & 5.9 & 2.1e-11 & 6.9e-12 & 5.4 & 4.5 & 6.5e-06 & 9.3e-06 & -6.8 & -9.3 & 2.1e-11 & 6.9e-12 & 5.4 & 4.6 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord2.tex <==
20& 2.62e-03 & 2.62e-03 & 2.02e-03 & 3.12 & 3.12 & 2.32 \\ 
40& 6.47e-04 & 6.47e-04 & 4.48e-04 & 2.02 & 2.02 & 2.17 \\ 
80& 1.57e-04 & 1.57e-04 & 9.06e-05 & 2.04 & 2.04 & 2.31 \\ 
160& 3.91e-05 & 3.91e-05 & 2.14e-05 & 2.01 & 2.01 & 2.08 \\ 
320& 9.77e-06 & 9.77e-06 & 5.29e-06 & 2.00 & 2.00 & 2.02 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord2_no_v.tex <==
20& 2.62e-03 & 2.02e-03 & 3.12 & 2.32 \\ 
40& 6.47e-04 & 4.48e-04 & 2.02 & 2.17 \\ 
80& 1.57e-04 & 9.06e-05 & 2.04 & 2.31 \\ 
160& 3.91e-05 & 2.14e-05 & 2.01 & 2.08 \\ 
320& 9.77e-06 & 5.29e-06 & 2.00 & 2.02 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord2_no_v_N.tex <==
 2.62e-03 & 2.02e-03 & 3.12 & 2.32 \\ 
 6.47e-04 & 4.48e-04 & 2.02 & 2.17 \\ 
 1.57e-04 & 9.06e-05 & 2.04 & 2.31 \\ 
 3.91e-05 & 2.14e-05 & 2.01 & 2.08 \\ 
 9.77e-06 & 5.29e-06 & 2.00 & 2.02 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord2a.tex <==
20& 2.62e-03 & 2.62e-03 & 2.02e-03 & 0.00 & 0.00 & 0.00 \\ 
40& 6.47e-04 & 6.47e-04 & 4.48e-04 & 2.02 & 2.02 & 2.17 \\ 
80& 1.57e-04 & 1.57e-04 & 9.06e-05 & 2.04 & 2.04 & 2.31 \\ 
160& 3.91e-05 & 3.91e-05 & 2.14e-05 & 2.01 & 2.01 & 2.08 \\ 
320& 9.77e-06 & 9.77e-06 & 5.29e-06 & 2.00 & 2.00 & 2.02 


==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord3.tex <==
10& 8.24e-04 & 8.24e-04 & 5.64e-04 & 4.33 & 4.33 & 4.46 \\ 
20& 1.41e-04 & 1.41e-04 & 8.98e-05 & 2.54 & 2.54 & 2.65 \\ 
40& 8.69e-06 & 8.69e-06 & 4.67e-06 & 4.02 & 4.02 & 4.27 \\ 
80& 5.27e-07 & 5.27e-07 & 2.16e-07 & 4.04 & 4.04 & 4.43 \\ 
160& 3.24e-08 & 3.24e-08 & 1.25e-08 & 4.03 & 4.03 & 4.11 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord3_no_v.tex <==
10& 8.24e-04 & 5.64e-04 & 4.33 & 4.46 \\ 
20& 1.41e-04 & 8.98e-05 & 2.54 & 2.65 \\ 
40& 8.69e-06 & 4.67e-06 & 4.02 & 4.27 \\ 
80& 5.27e-07 & 2.16e-07 & 4.04 & 4.43 \\ 
160& 3.24e-08 & 1.25e-08 & 4.03 & 4.11 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord3_no_v_N.tex <==
 8.24e-04 & 5.64e-04 & 4.33 & 4.46 \\ 
 1.41e-04 & 8.98e-05 & 2.54 & 2.65 \\ 
 8.69e-06 & 4.67e-06 & 4.02 & 4.27 \\ 
 5.27e-07 & 2.16e-07 & 4.04 & 4.43 \\ 
 3.24e-08 & 1.25e-08 & 4.03 & 4.11 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord3a.tex <==
10& 8.24e-04 & 8.24e-04 & 5.64e-04 & 0.00 & 0.00 & 0.00 \\ 
20& 1.41e-04 & 1.41e-04 & 8.98e-05 & 2.54 & 2.54 & 2.65 \\ 
40& 8.69e-06 & 8.69e-06 & 4.67e-06 & 4.02 & 4.02 & 4.27 \\ 
80& 5.27e-07 & 5.27e-07 & 2.16e-07 & 4.04 & 4.04 & 4.43 \\ 
160& 3.24e-08 & 3.24e-08 & 1.25e-08 & 4.03 & 4.03 & 4.11 


==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord4.tex <==
6& 1.39e-03 & 1.39e-03 & 2.77e-04 & 0.16 & 0.16 & 1.96 \\ 
13& 4.68e-05 & 4.68e-05 & 1.98e-05 & 4.39 & 4.39 & 3.41 \\ 
26& 1.97e-06 & 1.97e-06 & 4.49e-07 & 4.57 & 4.57 & 5.46 \\ 
53& 5.61e-08 & 5.61e-08 & 4.91e-09 & 5.00 & 5.00 & 6.34 \\ 
106& 1.74e-09 & 1.74e-09 & 8.82e-11 & 5.01 & 5.01 & 5.80 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord4_no_v.tex <==
6& 1.39e-03 & 2.77e-04 & 0.16 & 1.96 \\ 
13& 4.68e-05 & 1.98e-05 & 4.39 & 3.41 \\ 
26& 1.97e-06 & 4.49e-07 & 4.57 & 5.46 \\ 
53& 5.61e-08 & 4.91e-09 & 5.00 & 6.34 \\ 
106& 1.74e-09 & 8.82e-11 & 5.01 & 5.80 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord4_no_v_N.tex <==
 1.39e-03 & 2.77e-04 & 0.16 & 1.96 \\ 
 4.68e-05 & 1.98e-05 & 4.39 & 3.41 \\ 
 1.97e-06 & 4.49e-07 & 4.57 & 5.46 \\ 
 5.61e-08 & 4.91e-09 & 5.00 & 6.34 \\ 
 1.74e-09 & 8.82e-11 & 5.01 & 5.80 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord4a.tex <==
6& 1.39e-03 & 1.39e-03 & 2.77e-04 & 0.00 & 0.00 & 0.00 \\ 
13& 4.68e-05 & 4.68e-05 & 1.98e-05 & 4.39 & 4.39 & 3.41 \\ 
26& 1.97e-06 & 1.97e-06 & 4.49e-07 & 4.57 & 4.57 & 5.46 \\ 
53& 5.61e-08 & 5.61e-08 & 4.91e-09 & 5.00 & 5.00 & 6.34 \\ 
106& 1.74e-09 & 1.74e-09 & 8.82e-11 & 5.01 & 5.01 & 5.80 


==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord5.tex <==
5& 1.56e-03 & 1.56e-03 & 5.39e-04 & 2.94 & 2.94 & 2.61 \\ 
10& 9.52e-06 & 9.52e-06 & 2.36e-06 & 7.36 & 7.36 & 7.84 \\ 
20& 4.17e-07 & 4.17e-07 & 1.03e-07 & 4.51 & 4.51 & 4.52 \\ 
40& 6.62e-09 & 6.62e-09 & 1.07e-09 & 5.98 & 5.98 & 6.58 \\ 
80& 1.06e-10 & 1.06e-10 & 1.30e-11 & 5.97 & 5.97 & 6.36 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord51.tex <==
5& 2.42e-03 & 2.42e-03 & 2.22e-03 & 0.00 & 0.00 & 0.00 \\ 
10& 1.08e-05 & 1.08e-05 & 6.87e-06 & 7.82 & 7.82 & 8.34 \\ 
20& 4.64e-07 & 4.64e-07 & 2.56e-07 & 4.53 & 4.53 & 4.75 \\ 
40& 6.81e-09 & 6.81e-09 & 1.35e-09 & 6.09 & 6.09 & 7.57 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord51_no_v.tex <==
5& 2.42e-03 & 2.22e-03 & 0.00 & 0.00 \\ 
10& 1.08e-05 & 6.87e-06 & 7.82 & 8.34 \\ 
20& 4.64e-07 & 2.56e-07 & 4.53 & 4.75 \\ 
40& 6.81e-09 & 1.35e-09 & 6.09 & 7.57 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord51_no_v_N.tex <==
 2.42e-03 & 2.22e-03 & 0.00 & 0.00 \\ 
 1.08e-05 & 6.87e-06 & 7.82 & 8.34 \\ 
 4.64e-07 & 2.56e-07 & 4.53 & 4.75 \\ 
 6.81e-09 & 1.35e-09 & 6.09 & 7.57 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord5_no_v.tex <==
5& 1.56e-03 & 5.39e-04 & 2.94 & 2.61 \\ 
10& 9.52e-06 & 2.36e-06 & 7.36 & 7.84 \\ 
20& 4.17e-07 & 1.03e-07 & 4.51 & 4.52 \\ 
40& 6.62e-09 & 1.07e-09 & 5.98 & 6.58 \\ 
80& 1.06e-10 & 1.30e-11 & 5.97 & 6.36 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord5_no_v_N.tex <==
 1.56e-03 & 5.39e-04 & 2.94 & 2.61 \\ 
 9.52e-06 & 2.36e-06 & 7.36 & 7.84 \\ 
 4.17e-07 & 1.03e-07 & 4.51 & 4.52 \\ 
 6.62e-09 & 1.07e-09 & 5.98 & 6.58 \\ 
 1.06e-10 & 1.30e-11 & 5.97 & 6.36 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord5a.tex <==
5& 1.56e-03 & 1.56e-03 & 5.39e-04 & 0.00 & 0.00 & 0.00 \\ 
10& 9.52e-06 & 9.52e-06 & 2.36e-06 & 7.36 & 7.36 & 7.84 \\ 
20& 4.17e-07 & 4.17e-07 & 1.03e-07 & 4.51 & 4.51 & 4.52 \\ 
40& 6.62e-09 & 6.62e-09 & 1.07e-09 & 5.98 & 5.98 & 6.58 \\ 
80& 1.06e-10 & 1.06e-10 & 1.30e-11 & 5.97 & 5.97 & 6.36 


==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord6.tex <==
4& 9.24e-04 & 9.24e-04 & 3.18e-04 & 2.82 & 2.82 & 3.07 \\ 
8& 1.20e-05 & 1.20e-05 & 3.43e-06 & 6.27 & 6.27 & 6.53 \\ 
16& 1.24e-07 & 1.24e-07 & 2.19e-08 & 6.59 & 6.59 & 7.29 \\ 
32& 9.05e-10 & 9.05e-10 & 1.63e-10 & 7.10 & 7.10 & 7.07 \\ 
64& 2.12e-11 & 2.12e-11 & 6.88e-12 & 5.41 & 5.41 & 4.57 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord61.tex <==
4& 1.57e-03 & 1.57e-03 & 1.43e-03 & 0.00 & 0.00 & 0.00 \\ 
8& 1.50e-05 & 1.50e-05 & 1.15e-05 & 6.71 & 6.71 & 6.95 \\ 
16& 1.31e-07 & 1.31e-07 & 5.19e-08 & 6.83 & 6.83 & 7.79 \\ 
32& 1.19e-09 & 1.19e-09 & 7.93e-10 & 6.78 & 6.78 & 6.03 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord61_no_v.tex <==
4& 1.57e-03 & 1.43e-03 & 0.00 & 0.00 \\ 
8& 1.50e-05 & 1.15e-05 & 6.71 & 6.95 \\ 
16& 1.31e-07 & 5.19e-08 & 6.83 & 7.79 \\ 
32& 1.19e-09 & 7.93e-10 & 6.78 & 6.03 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord61_no_v_N.tex <==
 1.57e-03 & 1.43e-03 & 0.00 & 0.00 \\ 
 1.50e-05 & 1.15e-05 & 6.71 & 6.95 \\ 
 1.31e-07 & 5.19e-08 & 6.83 & 7.79 \\ 
 1.19e-09 & 7.93e-10 & 6.78 & 6.03 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord6_no_v.tex <==
4& 9.24e-04 & 3.18e-04 & 2.82 & 3.07 \\ 
8& 1.20e-05 & 3.43e-06 & 6.27 & 6.53 \\ 
16& 1.24e-07 & 2.19e-08 & 6.59 & 7.29 \\ 
32& 9.05e-10 & 1.63e-10 & 7.10 & 7.07 \\ 
64& 2.12e-11 & 6.88e-12 & 5.41 & 4.57 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord6_no_v_N.tex <==
 9.24e-04 & 3.18e-04 & 2.82 & 3.07 \\ 
 1.20e-05 & 3.43e-06 & 6.27 & 6.53 \\ 
 1.24e-07 & 2.19e-08 & 6.59 & 7.29 \\ 
 9.05e-10 & 1.63e-10 & 7.10 & 7.07 \\ 
 2.12e-11 & 6.88e-12 & 5.41 & 4.57 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord6a.tex <==
4& 9.24e-04 & 9.24e-04 & 3.18e-04 & 0.00 & 0.00 & 0.00 \\ 
8& 1.20e-05 & 1.20e-05 & 3.43e-06 & 6.27 & 6.27 & 6.53 \\ 
16& 1.24e-07 & 1.24e-07 & 2.19e-08 & 6.59 & 6.59 & 7.29 \\ 
32& 9.05e-10 & 9.05e-10 & 1.63e-10 & 7.10 & 7.10 & 7.07 \\ 
64& 2.12e-11 & 2.12e-11 & 6.88e-12 & 5.41 & 5.41 & 4.57 


==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord2.tex <==
20& 6.01e-03 & 6.01e-03 & 4.68e-03 & 0.00 & 0.00 & 0.00 \\ 
40& 1.33e-03 & 1.33e-03 & 9.05e-04 & 2.18 & 2.18 & 2.37 \\ 
80& 3.16e-04 & 3.16e-04 & 1.79e-04 & 2.07 & 2.07 & 2.33 \\ 
160& 7.83e-05 & 7.83e-05 & 4.21e-05 & 2.01 & 2.01 & 2.09 \\ 
320& 1.95e-05 & 1.95e-05 & 1.04e-05 & 2.00 & 2.00 & 2.02 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord2_no_v.tex <==
20& 6.01e-03 & 4.68e-03 & 0.00 & 0.00 \\ 
40& 1.33e-03 & 9.05e-04 & 2.18 & 2.37 \\ 
80& 3.16e-04 & 1.79e-04 & 2.07 & 2.33 \\ 
160& 7.83e-05 & 4.21e-05 & 2.01 & 2.09 \\ 
320& 1.95e-05 & 1.04e-05 & 2.00 & 2.02 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord2_no_v_N.tex <==
 6.01e-03 & 4.68e-03 & 0.00 & 0.00 \\ 
 1.33e-03 & 9.05e-04 & 2.18 & 2.37 \\ 
 3.16e-04 & 1.79e-04 & 2.07 & 2.33 \\ 
 7.83e-05 & 4.21e-05 & 2.01 & 2.09 \\ 
 1.95e-05 & 1.04e-05 & 2.00 & 2.02 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord3.tex <==
10& 9.03e-03 & 9.03e-03 & 5.70e-03 & 0.00 & 0.00 & 0.00 \\ 
20& 2.15e-03 & 2.15e-03 & 1.24e-03 & 2.07 & 2.07 & 2.20 \\ 
40& 6.19e-04 & 6.19e-04 & 2.51e-04 & 1.80 & 1.80 & 2.31 \\ 
80& 1.78e-04 & 1.78e-04 & 4.13e-05 & 1.80 & 1.80 & 2.60 \\ 
160& 4.78e-05 & 4.78e-05 & 8.75e-06 & 1.90 & 1.90 & 2.24 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord3_no_v.tex <==
10& 9.03e-03 & 5.70e-03 & 0.00 & 0.00 \\ 
20& 2.15e-03 & 1.24e-03 & 2.07 & 2.20 \\ 
40& 6.19e-04 & 2.51e-04 & 1.80 & 2.31 \\ 
80& 1.78e-04 & 4.13e-05 & 1.80 & 2.60 \\ 
160& 4.78e-05 & 8.75e-06 & 1.90 & 2.24 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord3_no_v_N.tex <==
 9.03e-03 & 5.70e-03 & 0.00 & 0.00 \\ 
 2.15e-03 & 1.24e-03 & 2.07 & 2.20 \\ 
 6.19e-04 & 2.51e-04 & 1.80 & 2.31 \\ 
 1.78e-04 & 4.13e-05 & 1.80 & 2.60 \\ 
 4.78e-05 & 8.75e-06 & 1.90 & 2.24 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord4.tex <==
6& 1.39e-02 & 1.39e-02 & 1.02e-02 & 0.00 & 0.00 & 0.00 \\ 
13& 2.51e-03 & 2.51e-03 & 1.68e-03 & 2.21 & 2.21 & 2.33 \\ 
26& 3.83e-05 & 3.83e-05 & 6.73e-06 & 6.03 & 6.03 & 7.96 \\ 
53& 1.76e-06 & 1.76e-06 & 2.34e-07 & 4.32 & 4.32 & 4.72 \\ 
106& 1.04e-07 & 1.04e-07 & 1.07e-08 & 4.08 & 4.08 & 4.45 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord4_no_v.tex <==
6& 1.39e-02 & 1.02e-02 & 0.00 & 0.00 \\ 
13& 2.51e-03 & 1.68e-03 & 2.21 & 2.33 \\ 
26& 3.83e-05 & 6.73e-06 & 6.03 & 7.96 \\ 
53& 1.76e-06 & 2.34e-07 & 4.32 & 4.72 \\ 
106& 1.04e-07 & 1.07e-08 & 4.08 & 4.45 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord4_no_v_N.tex <==
 1.39e-02 & 1.02e-02 & 0.00 & 0.00 \\ 
 2.51e-03 & 1.68e-03 & 2.21 & 2.33 \\ 
 3.83e-05 & 6.73e-06 & 6.03 & 7.96 \\ 
 1.76e-06 & 2.34e-07 & 4.32 & 4.72 \\ 
 1.04e-07 & 1.07e-08 & 4.08 & 4.45 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord5.tex <==
5& 2.81e-03 & 2.81e-03 & 1.29e-03 & 0.00 & 0.00 & 0.00 \\ 
10& 2.95e-04 & 2.95e-04 & 6.99e-05 & 3.26 & 3.26 & 4.21 \\ 
20& 1.45e-05 & 1.45e-05 & 4.27e-06 & 4.35 & 4.35 & 4.04 \\ 
40& 1.16e-06 & 1.16e-06 & 1.86e-07 & 3.65 & 3.65 & 4.52 \\ 
80& 8.61e-08 & 8.61e-08 & 3.78e-08 & 3.75 & 3.75 & 2.30 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord51.tex <==
5& 2.81e-03 & 2.81e-03 & 1.29e-03 & 0.00 & 0.00 & 0.00 \\ 
10& 2.95e-04 & 2.95e-04 & 6.99e-05 & 3.26 & 3.26 & 4.21 \\ 
20& 1.45e-05 & 1.45e-05 & 4.27e-06 & 4.35 & 4.35 & 4.04 \\ 
40& 1.16e-06 & 1.16e-06 & 1.86e-07 & 3.65 & 3.65 & 4.52 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord51_no_v.tex <==
5& 2.81e-03 & 1.29e-03 & 0.00 & 0.00 \\ 
10& 2.95e-04 & 6.99e-05 & 3.26 & 4.21 \\ 
20& 1.45e-05 & 4.27e-06 & 4.35 & 4.04 \\ 
40& 1.16e-06 & 1.86e-07 & 3.65 & 4.52 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord51_no_v_N.tex <==
 2.81e-03 & 1.29e-03 & 0.00 & 0.00 \\ 
 2.95e-04 & 6.99e-05 & 3.26 & 4.21 \\ 
 1.45e-05 & 4.27e-06 & 4.35 & 4.04 \\ 
 1.16e-06 & 1.86e-07 & 3.65 & 4.52 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord5_no_v.tex <==
5& 2.81e-03 & 1.29e-03 & 0.00 & 0.00 \\ 
10& 2.95e-04 & 6.99e-05 & 3.26 & 4.21 \\ 
20& 1.45e-05 & 4.27e-06 & 4.35 & 4.04 \\ 
40& 1.16e-06 & 1.86e-07 & 3.65 & 4.52 \\ 
80& 8.61e-08 & 3.78e-08 & 3.75 & 2.30 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord5_no_v_N.tex <==
 2.81e-03 & 1.29e-03 & 0.00 & 0.00 \\ 
 2.95e-04 & 6.99e-05 & 3.26 & 4.21 \\ 
 1.45e-05 & 4.27e-06 & 4.35 & 4.04 \\ 
 1.16e-06 & 1.86e-07 & 3.65 & 4.52 \\ 
 8.61e-08 & 3.78e-08 & 3.75 & 2.30 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord6.tex <==
4& 6.12e-03 & 6.12e-03 & 2.97e-03 & 0.00 & 0.00 & 0.00 \\ 
8& 3.01e-04 & 3.01e-04 & 1.55e-04 & 4.35 & 4.35 & 4.26 \\ 
16& 6.36e-06 & 6.36e-06 & 1.64e-06 & 5.56 & 5.56 & 6.56 \\ 
32& 5.81e-08 & 5.81e-08 & 1.52e-08 & 6.77 & 6.77 & 6.76 \\ 
64& 6.55e-06 & 6.55e-06 & 9.26e-06 & -6.82 & -6.82 & -9.26 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord61.tex <==
4& 6.12e-03 & 6.12e-03 & 2.97e-03 & 0.00 & 0.00 & 0.00 \\ 
8& 3.01e-04 & 3.01e-04 & 1.55e-04 & 4.35 & 4.35 & 4.26 \\ 
16& 6.36e-06 & 6.36e-06 & 1.64e-06 & 5.56 & 5.56 & 6.56 \\ 
32& 5.81e-08 & 5.81e-08 & 1.52e-08 & 6.77 & 6.77 & 6.76 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord61_no_v.tex <==
4& 6.12e-03 & 2.97e-03 & 0.00 & 0.00 \\ 
8& 3.01e-04 & 1.55e-04 & 4.35 & 4.26 \\ 
16& 6.36e-06 & 1.64e-06 & 5.56 & 6.56 \\ 
32& 5.81e-08 & 1.52e-08 & 6.77 & 6.76 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord61_no_v_N.tex <==
 6.12e-03 & 2.97e-03 & 0.00 & 0.00 \\ 
 3.01e-04 & 1.55e-04 & 4.35 & 4.26 \\ 
 6.36e-06 & 1.64e-06 & 5.56 & 6.56 \\ 
 5.81e-08 & 1.52e-08 & 6.77 & 6.76 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord6_no_v.tex <==
4& 6.12e-03 & 2.97e-03 & 0.00 & 0.00 \\ 
8& 3.01e-04 & 1.55e-04 & 4.35 & 4.26 \\ 
16& 6.36e-06 & 1.64e-06 & 5.56 & 6.56 \\ 
32& 5.81e-08 & 1.52e-08 & 6.77 & 6.76 \\ 
64& 6.55e-06 & 9.26e-06 & -6.82 & -9.26 

==> figures/LinAc2D_coriolis_vortex/errors_OSS_ord6_no_v_N.tex <==
 6.12e-03 & 2.97e-03 & 0.00 & 0.00 \\ 
 3.01e-04 & 1.55e-04 & 4.35 & 4.26 \\ 
 6.36e-06 & 1.64e-06 & 5.56 & 6.56 \\ 
 5.81e-08 & 1.52e-08 & 6.77 & 6.76 \\ 
 6.55e-06 & 9.26e-06 & -6.82 & -9.26 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_GF_ord2.tex <==
20& 2.53e-03 & 2.53e-03 & 1.65e-03 & 0.00 & 0.00 & 0.00 \\ 
40& 6.39e-04 & 6.39e-04 & 4.21e-04 & 1.99 & 1.99 & 1.97 \\ 
80& 1.57e-04 & 1.57e-04 & 8.91e-05 & 2.03 & 2.03 & 2.24 \\ 
160& 3.91e-05 & 3.91e-05 & 2.14e-05 & 2.00 & 2.00 & 2.06 \\ 
320& 9.77e-06 & 9.77e-06 & 5.29e-06 & 2.00 & 2.00 & 2.01 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_GF_ord2_no_v.tex <==
20& 2.53e-03 & 1.65e-03 & 0.00 & 0.00 \\ 
40& 6.39e-04 & 4.21e-04 & 1.99 & 1.97 \\ 
80& 1.57e-04 & 8.91e-05 & 2.03 & 2.24 \\ 
160& 3.91e-05 & 2.14e-05 & 2.00 & 2.06 \\ 
320& 9.77e-06 & 5.29e-06 & 2.00 & 2.01 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_GF_ord2_no_v_N.tex <==
 2.53e-03 & 1.65e-03 & 0.00 & 0.00 \\ 
 6.39e-04 & 4.21e-04 & 1.99 & 1.97 \\ 
 1.57e-04 & 8.91e-05 & 2.03 & 2.24 \\ 
 3.91e-05 & 2.14e-05 & 2.00 & 2.06 \\ 
 9.77e-06 & 5.29e-06 & 2.00 & 2.01 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_GF_ord3.tex <==
10& 7.65e-04 & 7.65e-04 & 2.51e-04 & 0.00 & 0.00 & 0.00 \\ 
20& 1.31e-04 & 1.31e-04 & 5.06e-05 & 2.55 & 2.55 & 2.31 \\ 
40& 8.19e-06 & 8.19e-06 & 3.16e-06 & 4.00 & 4.00 & 4.00 \\ 
80& 5.06e-07 & 5.06e-07 & 1.98e-07 & 4.02 & 4.02 & 4.00 \\ 
160& 3.15e-08 & 3.15e-08 & 1.24e-08 & 4.01 & 4.01 & 4.00 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_GF_ord3_no_v.tex <==
10& 7.65e-04 & 2.51e-04 & 0.00 & 0.00 \\ 
20& 1.31e-04 & 5.06e-05 & 2.55 & 2.31 \\ 
40& 8.19e-06 & 3.16e-06 & 4.00 & 4.00 \\ 
80& 5.06e-07 & 1.98e-07 & 4.02 & 4.00 \\ 
160& 3.15e-08 & 1.24e-08 & 4.01 & 4.00 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_GF_ord3_no_v_N.tex <==
 7.65e-04 & 2.51e-04 & 0.00 & 0.00 \\ 
 1.31e-04 & 5.06e-05 & 2.55 & 2.31 \\ 
 8.19e-06 & 3.16e-06 & 4.00 & 4.00 \\ 
 5.06e-07 & 1.98e-07 & 4.02 & 4.00 \\ 
 3.15e-08 & 1.24e-08 & 4.01 & 4.00 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_GF_ord4.tex <==
6& 1.38e-03 & 1.38e-03 & 2.24e-04 & 0.00 & 0.00 & 0.00 \\ 
13& 4.64e-05 & 4.64e-05 & 1.88e-05 & 4.39 & 4.39 & 3.20 \\ 
26& 1.97e-06 & 1.97e-06 & 4.14e-07 & 4.56 & 4.56 & 5.50 \\ 
53& 5.61e-08 & 5.61e-08 & 4.26e-09 & 4.99 & 4.99 & 6.43 \\ 
106& 1.74e-09 & 1.74e-09 & 7.92e-11 & 5.01 & 5.01 & 5.75 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_GF_ord4_no_v.tex <==
6& 1.38e-03 & 2.24e-04 & 0.00 & 0.00 \\ 
13& 4.64e-05 & 1.88e-05 & 4.39 & 3.20 \\ 
26& 1.97e-06 & 4.14e-07 & 4.56 & 5.50 \\ 
53& 5.61e-08 & 4.26e-09 & 4.99 & 6.43 \\ 
106& 1.74e-09 & 7.92e-11 & 5.01 & 5.75 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_GF_ord4_no_v_N.tex <==
 1.38e-03 & 2.24e-04 & 0.00 & 0.00 \\ 
 4.64e-05 & 1.88e-05 & 4.39 & 3.20 \\ 
 1.97e-06 & 4.14e-07 & 4.56 & 5.50 \\ 
 5.61e-08 & 4.26e-09 & 4.99 & 6.43 \\ 
 1.74e-09 & 7.92e-11 & 5.01 & 5.75 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_GF_ord5.tex <==
5& 1.56e-03 & 1.56e-03 & 4.93e-04 & 0.00 & 0.00 & 0.00 \\ 
10& 9.50e-06 & 9.50e-06 & 2.37e-06 & 7.36 & 7.36 & 7.70 \\ 
20& 4.16e-07 & 4.16e-07 & 1.02e-07 & 4.51 & 4.51 & 4.54 \\ 
40& 6.60e-09 & 6.60e-09 & 9.54e-10 & 5.98 & 5.98 & 6.73 \\ 
80& 1.05e-10 & 1.05e-10 & 1.16e-11 & 5.97 & 5.97 & 6.36 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_GF_ord5_no_v.tex <==
5& 1.56e-03 & 4.93e-04 & 0.00 & 0.00 \\ 
10& 9.50e-06 & 2.37e-06 & 7.36 & 7.70 \\ 
20& 4.16e-07 & 1.02e-07 & 4.51 & 4.54 \\ 
40& 6.60e-09 & 9.54e-10 & 5.98 & 6.73 \\ 
80& 1.05e-10 & 1.16e-11 & 5.97 & 6.36 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_GF_ord5_no_v_N.tex <==
 1.56e-03 & 4.93e-04 & 0.00 & 0.00 \\ 
 9.50e-06 & 2.37e-06 & 7.36 & 7.70 \\ 
 4.16e-07 & 1.02e-07 & 4.51 & 4.54 \\ 
 6.60e-09 & 9.54e-10 & 5.98 & 6.73 \\ 
 1.05e-10 & 1.16e-11 & 5.97 & 6.36 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_GF_ord6.tex <==
4& 9.19e-04 & 9.19e-04 & 2.67e-04 & 0.00 & 0.00 & 0.00 \\ 
8& 1.19e-05 & 1.19e-05 & 3.06e-06 & 6.27 & 6.27 & 6.45 \\ 
16& 1.24e-07 & 1.24e-07 & 1.81e-08 & 6.59 & 6.59 & 7.41 \\ 
32& 9.03e-10 & 9.03e-10 & 1.59e-10 & 7.10 & 7.10 & 6.83 \\ 
64& 2.13e-11 & 2.13e-11 & 6.90e-12 & 5.41 & 5.41 & 4.52 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_GF_ord6_no_v.tex <==
4& 9.19e-04 & 2.67e-04 & 0.00 & 0.00 \\ 
8& 1.19e-05 & 3.06e-06 & 6.27 & 6.45 \\ 
16& 1.24e-07 & 1.81e-08 & 6.59 & 7.41 \\ 
32& 9.03e-10 & 1.59e-10 & 7.10 & 6.83 \\ 
64& 2.13e-11 & 6.90e-12 & 5.41 & 4.52 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_GF_ord6_no_v_N.tex <==
 9.19e-04 & 2.67e-04 & 0.00 & 0.00 \\ 
 1.19e-05 & 3.06e-06 & 6.27 & 6.45 \\ 
 1.24e-07 & 1.81e-08 & 6.59 & 7.41 \\ 
 9.03e-10 & 1.59e-10 & 7.10 & 6.83 \\ 
 2.13e-11 & 6.90e-12 & 5.41 & 4.52 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_GF_ord7.tex <==
3& 2.45e-03 & 2.45e-03 & 1.01e-03 & 0.00 & 0.00 & 0.00 \\ 
6& 1.88e-05 & 1.88e-05 & 4.57e-06 & 7.03 & 7.03 & 7.78 \\ 
13& 5.73e-08 & 5.73e-08 & 1.43e-08 & 7.49 & 7.49 & 7.46 \\ 
26& 1.67e-10 & 1.67e-10 & 2.63e-11 & 8.42 & 8.42 & 9.09 \\ 
53& 1.97e-11 & 1.97e-11 & 6.75e-12 & 3.00 & 3.00 & 1.91 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_GF_ord7_no_v.tex <==
3& 2.45e-03 & 1.01e-03 & 0.00 & 0.00 \\ 
6& 1.88e-05 & 4.57e-06 & 7.03 & 7.78 \\ 
13& 5.73e-08 & 1.43e-08 & 7.49 & 7.46 \\ 
26& 1.67e-10 & 2.63e-11 & 8.42 & 9.09 \\ 
53& 1.97e-11 & 6.75e-12 & 3.00 & 1.91 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_GF_ord7_no_v_N.tex <==
 2.45e-03 & 1.01e-03 & 0.00 & 0.00 \\ 
 1.88e-05 & 4.57e-06 & 7.03 & 7.78 \\ 
 5.73e-08 & 1.43e-08 & 7.49 & 7.46 \\ 
 1.67e-10 & 2.63e-11 & 8.42 & 9.09 \\ 
 1.97e-11 & 6.75e-12 & 3.00 & 1.91 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_ord2.tex <==
20& 7.90e-03 & 7.90e-03 & 3.86e-03 & 0.00 & 0.00 & 0.00 \\ 
40& 1.57e-03 & 1.57e-03 & 8.55e-04 & 2.33 & 2.33 & 2.18 \\ 
80& 3.37e-04 & 3.37e-04 & 1.77e-04 & 2.22 & 2.22 & 2.27 \\ 
160& 7.97e-05 & 7.97e-05 & 4.25e-05 & 2.08 & 2.08 & 2.06 \\ 
320& 1.96e-05 & 1.96e-05 & 1.05e-05 & 2.02 & 2.02 & 2.01 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_ord2_no_v.tex <==
20& 7.90e-03 & 3.86e-03 & 0.00 & 0.00 \\ 
40& 1.57e-03 & 8.55e-04 & 2.33 & 2.18 \\ 
80& 3.37e-04 & 1.77e-04 & 2.22 & 2.27 \\ 
160& 7.97e-05 & 4.25e-05 & 2.08 & 2.06 \\ 
320& 1.96e-05 & 1.05e-05 & 2.02 & 2.01 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_ord2_no_v_N.tex <==
 7.90e-03 & 3.86e-03 & 0.00 & 0.00 \\ 
 1.57e-03 & 8.55e-04 & 2.33 & 2.18 \\ 
 3.37e-04 & 1.77e-04 & 2.22 & 2.27 \\ 
 7.97e-05 & 4.25e-05 & 2.08 & 2.06 \\ 
 1.96e-05 & 1.05e-05 & 2.02 & 2.01 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_ord3.tex <==
10& 1.13e-02 & 1.13e-02 & 3.13e-03 & 0.00 & 0.00 & 0.00 \\ 
20& 2.90e-03 & 2.90e-03 & 4.91e-04 & 1.96 & 1.96 & 2.67 \\ 
40& 7.78e-04 & 7.78e-04 & 1.34e-04 & 1.90 & 1.90 & 1.87 \\ 
80& 1.73e-04 & 1.73e-04 & 2.94e-05 & 2.17 & 2.17 & 2.19 \\ 
160& 3.25e-05 & 3.25e-05 & 5.23e-06 & 2.42 & 2.42 & 2.49 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_ord3_no_v.tex <==
10& 1.13e-02 & 3.13e-03 & 0.00 & 0.00 \\ 
20& 2.90e-03 & 4.91e-04 & 1.96 & 2.67 \\ 
40& 7.78e-04 & 1.34e-04 & 1.90 & 1.87 \\ 
80& 1.73e-04 & 2.94e-05 & 2.17 & 2.19 \\ 
160& 3.25e-05 & 5.23e-06 & 2.42 & 2.49 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_ord3_no_v_N.tex <==
 1.13e-02 & 3.13e-03 & 0.00 & 0.00 \\ 
 2.90e-03 & 4.91e-04 & 1.96 & 2.67 \\ 
 7.78e-04 & 1.34e-04 & 1.90 & 1.87 \\ 
 1.73e-04 & 2.94e-05 & 2.17 & 2.19 \\ 
 3.25e-05 & 5.23e-06 & 2.42 & 2.49 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_ord4.tex <==
6& 1.10e-02 & 1.10e-02 & 2.22e-03 & 0.00 & 0.00 & 0.00 \\ 
13& 1.58e-03 & 1.58e-03 & 2.75e-04 & 2.51 & 2.51 & 2.70 \\ 
26& 8.26e-05 & 8.26e-05 & 1.18e-05 & 4.26 & 4.26 & 4.54 \\ 
53& 4.29e-06 & 4.29e-06 & 6.02e-07 & 4.15 & 4.15 & 4.18 \\ 
106& 2.62e-07 & 2.62e-07 & 3.65e-08 & 4.03 & 4.03 & 4.04 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_ord4_no_v.tex <==
6& 1.10e-02 & 2.22e-03 & 0.00 & 0.00 \\ 
13& 1.58e-03 & 2.75e-04 & 2.51 & 2.70 \\ 
26& 8.26e-05 & 1.18e-05 & 4.26 & 4.54 \\ 
53& 4.29e-06 & 6.02e-07 & 4.15 & 4.18 \\ 
106& 2.62e-07 & 3.65e-08 & 4.03 & 4.04 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_ord4_no_v_N.tex <==
 1.10e-02 & 2.22e-03 & 0.00 & 0.00 \\ 
 1.58e-03 & 2.75e-04 & 2.51 & 2.70 \\ 
 8.26e-05 & 1.18e-05 & 4.26 & 4.54 \\ 
 4.29e-06 & 6.02e-07 & 4.15 & 4.18 \\ 
 2.62e-07 & 3.65e-08 & 4.03 & 4.04 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_ord5.tex <==
5& 2.00e-03 & 2.00e-03 & 5.81e-04 & 0.00 & 0.00 & 0.00 \\ 
10& 5.39e-04 & 5.39e-04 & 7.62e-05 & 1.89 & 1.89 & 2.93 \\ 
20& 2.27e-05 & 2.27e-05 & 2.89e-06 & 4.57 & 4.57 & 4.72 \\ 
40& 1.18e-06 & 1.18e-06 & 1.38e-07 & 4.27 & 4.27 & 4.39 \\ 
80& 4.92e-08 & 4.92e-08 & 5.54e-09 & 4.58 & 4.58 & 4.64 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_ord5_no_v.tex <==
5& 2.00e-03 & 5.81e-04 & 0.00 & 0.00 \\ 
10& 5.39e-04 & 7.62e-05 & 1.89 & 2.93 \\ 
20& 2.27e-05 & 2.89e-06 & 4.57 & 4.72 \\ 
40& 1.18e-06 & 1.38e-07 & 4.27 & 4.39 \\ 
80& 4.92e-08 & 5.54e-09 & 4.58 & 4.64 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_ord5_no_v_N.tex <==
 2.00e-03 & 5.81e-04 & 0.00 & 0.00 \\ 
 5.39e-04 & 7.62e-05 & 1.89 & 2.93 \\ 
 2.27e-05 & 2.89e-06 & 4.57 & 4.72 \\ 
 1.18e-06 & 1.38e-07 & 4.27 & 4.39 \\ 
 4.92e-08 & 5.54e-09 & 4.58 & 4.64 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_ord6.tex <==
4& 5.11e-03 & 5.11e-03 & 6.49e-04 & 0.00 & 0.00 & 0.00 \\ 
8& 2.05e-04 & 2.05e-04 & 2.35e-05 & 4.64 & 4.64 & 4.79 \\ 
16& 6.16e-06 & 6.16e-06 & 6.17e-07 & 5.06 & 5.06 & 5.25 \\ 
32& 1.11e-07 & 1.11e-07 & 1.20e-08 & 5.79 & 5.79 & 5.69 \\ 
64& 1.75e-09 & 1.75e-09 & 2.04e-10 & 5.99 & 5.99 & 5.88 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_ord6_no_v.tex <==
4& 5.11e-03 & 6.49e-04 & 0.00 & 0.00 \\ 
8& 2.05e-04 & 2.35e-05 & 4.64 & 4.79 \\ 
16& 6.16e-06 & 6.17e-07 & 5.06 & 5.25 \\ 
32& 1.11e-07 & 1.20e-08 & 5.79 & 5.69 \\ 
64& 1.75e-09 & 2.04e-10 & 5.99 & 5.88 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_ord6_no_v_N.tex <==
 5.11e-03 & 6.49e-04 & 0.00 & 0.00 \\ 
 2.05e-04 & 2.35e-05 & 4.64 & 4.79 \\ 
 6.16e-06 & 6.17e-07 & 5.06 & 5.25 \\ 
 1.11e-07 & 1.20e-08 & 5.79 & 5.69 \\ 
 1.75e-09 & 2.04e-10 & 5.99 & 5.88 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_ord7.tex <==
3& 2.44e-03 & 2.44e-03 & 9.56e-04 & 0.00 & 0.00 & 0.00 \\ 
6& 4.19e-05 & 4.19e-05 & 1.04e-05 & 5.87 & 5.87 & 6.52 \\ 
13& 4.44e-07 & 4.44e-07 & 6.62e-08 & 5.88 & 5.88 & 6.54 \\ 
26& 2.01e-08 & 2.01e-08 & 2.72e-09 & 4.47 & 4.47 & 4.61 \\ 
53& 2.23e-10 & 2.23e-10 & 2.97e-11 & 6.32 & 6.32 & 6.34 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_ord7_no_v.tex <==
3& 2.44e-03 & 9.56e-04 & 0.00 & 0.00 \\ 
6& 4.19e-05 & 1.04e-05 & 5.87 & 6.52 \\ 
13& 4.44e-07 & 6.62e-08 & 5.88 & 6.54 \\ 
26& 2.01e-08 & 2.72e-09 & 4.47 & 4.61 \\ 
53& 2.23e-10 & 2.97e-11 & 6.32 & 6.34 

==> figures/LinAc2D_coriolis_vortex/errors_SUPG_ord7_no_v_N.tex <==
 2.44e-03 & 9.56e-04 & 0.00 & 0.00 \\ 
 4.19e-05 & 1.04e-05 & 5.87 & 6.52 \\ 
 4.44e-07 & 6.62e-08 & 5.88 & 6.54 \\ 
 2.01e-08 & 2.72e-09 & 4.47 & 4.61 \\ 
 2.23e-10 & 2.97e-11 & 6.32 & 6.34 

==> figures/LinAc2D_moving_source/big_table_ord2.tex <==
10 & 2.1e-04 & 9.1e-04 & 0.0 & 0.0 & 8.0e-05 & 1.6e-04 & 0.0 & 0.0 & 2.3e-04 & 9.5e-04 & 0.0 & 0.0 & 6.5e-05 & 1.7e-04 & 0.0 & 0.0 \\
20 & 1.3e-04 & 2.5e-04 & 0.8 & 1.9 & 5.5e-05 & 8.7e-05 & 0.5 & 0.9 & 1.4e-04 & 2.4e-04 & 0.7 & 2.0 & 5.4e-05 & 9.0e-05 & 0.3 & 0.9 \\
40 & 4.1e-05 & 5.4e-05 & 1.6 & 2.2 & 2.0e-05 & 2.4e-05 & 1.5 & 1.9 & 4.3e-05 & 5.3e-05 & 1.7 & 2.2 & 2.0e-05 & 2.4e-05 & 1.5 & 1.9 \\
80 & 1.1e-05 & 1.3e-05 & 1.9 & 2.1 & 5.2e-06 & 5.9e-06 & 1.9 & 2.0 & 1.1e-05 & 1.3e-05 & 2.0 & 2.1 & 5.2e-06 & 5.9e-06 & 1.9 & 2.0 \\
160 & 2.7e-06 & 3.2e-06 & 2.0 & 2.0 & 1.3e-06 & 1.5e-06 & 2.0 & 2.0 & 2.8e-06 & 3.1e-06 & 2.0 & 2.0 & 1.3e-06 & 1.5e-06 & 2.0 & 2.0 

==> figures/LinAc2D_moving_source/big_table_ord3.tex <==
5 & 2.7e-04 & 7.0e-04 & 0.0 & 0.0 & 2.4e-04 & 4.9e-04 & 0.0 & 0.0 & 2.7e-04 & 7.7e-04 & 0.0 & 0.0 & 2.0e-04 & 5.2e-04 & 0.0 & 0.0 \\
10 & 1.8e-04 & 1.6e-04 & 0.6 & 2.1 & 4.0e-05 & 6.9e-05 & 2.6 & 2.8 & 2.1e-04 & 1.5e-04 & 0.3 & 2.3 & 4.0e-05 & 7.3e-05 & 2.3 & 2.8 \\
20 & 3.1e-05 & 2.9e-05 & 2.6 & 2.5 & 5.3e-06 & 6.0e-06 & 2.9 & 3.5 & 4.3e-05 & 3.4e-05 & 2.3 & 2.2 & 5.9e-06 & 8.2e-06 & 2.8 & 3.2 \\
40 & 5.1e-06 & 6.7e-06 & 2.6 & 2.1 & 6.8e-07 & 7.4e-07 & 2.9 & 3.0 & 9.5e-06 & 7.2e-06 & 2.2 & 2.2 & 9.0e-07 & 1.5e-06 & 2.7 & 2.4 \\
80 & 7.1e-07 & 1.3e-06 & 2.8 & 2.3 & 1.1e-07 & 8.3e-08 & 2.6 & 3.1 & 2.0e-06 & 1.7e-06 & 2.3 & 2.1 & 1.9e-07 & 3.0e-07 & 2.3 & 2.3 

==> figures/LinAc2D_moving_source/big_table_ord4.tex <==
3 & 2.9e-04 & 8.0e-04 & 0.0 & 0.0 & 2.8e-04 & 6.4e-04 & 0.0 & 0.0 & 2.9e-04 & 8.5e-04 & 0.0 & 0.0 & 2.5e-04 & 6.6e-04 & 0.0 & 0.0 \\
6 & 1.7e-04 & 2.2e-04 & 0.7 & 1.8 & 6.9e-05 & 6.8e-05 & 2.0 & 3.2 & 1.9e-04 & 2.5e-04 & 0.6 & 1.7 & 6.9e-05 & 7.2e-05 & 1.9 & 3.2 \\
13 & 9.5e-06 & 1.7e-05 & 3.7 & 3.3 & 2.7e-06 & 1.9e-06 & 4.2 & 4.6 & 1.0e-05 & 2.0e-05 & 3.8 & 3.3 & 2.7e-06 & 2.0e-06 & 4.2 & 4.6 \\
26 & 6.6e-07 & 6.0e-07 & 3.9 & 4.8 & 9.3e-08 & 1.1e-07 & 4.8 & 4.2 & 7.7e-07 & 6.5e-07 & 3.7 & 4.9 & 9.5e-08 & 1.2e-07 & 4.8 & 4.1 \\
53 & 3.8e-08 & 2.4e-08 & 4.0 & 4.5 & 5.6e-09 & 6.5e-09 & 3.9 & 3.9 & 4.4e-08 & 2.5e-08 & 4.0 & 4.6 & 5.5e-09 & 7.3e-09 & 4.0 & 4.0 

==> figures/LinAc2D_moving_source/big_table_ord5.tex <==
2 & 6.7e-04 & 9.8e-04 & 0.0 & 0.0 & 5.7e-04 & 7.8e-04 & 0.0 & 0.0 & 6.7e-04 & 1.0e-03 & 0.0 & 0.0 & 5.4e-04 & 8.1e-04 & 0.0 & 0.0 \\
5 & 7.3e-05 & 9.9e-05 & 2.4 & 2.5 & 4.7e-05 & 3.4e-05 & 2.7 & 3.4 & 6.8e-05 & 1.2e-04 & 2.5 & 2.4 & 4.7e-05 & 3.5e-05 & 2.7 & 3.4 \\
10 & 3.8e-06 & 3.5e-06 & 4.3 & 4.8 & 7.5e-07 & 7.4e-07 & 6.0 & 5.5 & 5.2e-06 & 4.2e-06 & 3.7 & 4.8 & 7.9e-07 & 8.9e-07 & 5.9 & 5.3 \\
20 & 1.2e-07 & 1.5e-07 & 4.9 & 4.6 & 2.2e-08 & 1.8e-08 & 5.1 & 5.3 & 1.5e-07 & 1.9e-07 & 5.1 & 4.5 & 2.3e-08 & 2.3e-08 & 5.1 & 5.3 \\
40 & 5.9e-09 & 7.2e-09 & 4.4 & 4.4 & 3.9e-09 & 2.7e-09 & 2.5 & 2.7 & 6.0e-09 & 9.0e-09 & 4.7 & 4.4 & 3.9e-09 & 2.7e-09 & 2.6 & 3.1 

==> figures/LinAc2D_moving_source/errors_OSS_GF_ord2.tex <==
10& 6.51e-05 & 9.26e-05 & 1.67e-04 & 0.00 & 0.00 & 0.00 \\ 
20& 5.42e-05 & 5.42e-05 & 9.02e-05 & 0.26 & 0.77 & 0.89 \\ 
40& 1.96e-05 & 1.96e-05 & 2.37e-05 & 1.47 & 1.47 & 1.93 \\ 
80& 5.21e-06 & 5.21e-06 & 5.94e-06 & 1.91 & 1.91 & 2.00 \\ 
160& 1.32e-06 & 1.32e-06 & 1.49e-06 & 1.98 & 1.98 & 2.00 

==> figures/LinAc2D_moving_source/errors_OSS_GF_ord3.tex <==
5& 2.02e-04 & 1.53e-04 & 5.18e-04 & 0.00 & 0.00 & 0.00 \\ 
10& 4.02e-05 & 7.21e-05 & 7.34e-05 & 2.33 & 1.09 & 2.82 \\ 
20& 5.89e-06 & 5.89e-06 & 8.17e-06 & 2.77 & 3.61 & 3.17 \\ 
40& 9.01e-07 & 9.01e-07 & 1.50e-06 & 2.71 & 2.71 & 2.44 \\ 
80& 1.89e-07 & 1.89e-07 & 2.97e-07 & 2.25 & 2.25 & 2.34 

==> figures/LinAc2D_moving_source/errors_OSS_GF_ord4.tex <==
3& 2.54e-04 & 2.98e-04 & 6.56e-04 & 0.00 & 0.00 & 0.00 \\ 
6& 6.91e-05 & 8.60e-05 & 7.15e-05 & 1.88 & 1.79 & 3.20 \\ 
13& 2.72e-06 & 2.62e-06 & 2.04e-06 & 4.18 & 4.51 & 4.60 \\ 
26& 9.47e-08 & 9.46e-08 & 1.23e-07 & 4.84 & 4.79 & 4.05 \\ 
53& 5.53e-09 & 4.01e-09 & 7.34e-09 & 3.99 & 4.44 & 3.95 

==> figures/LinAc2D_moving_source/errors_OSS_GF_ord5.tex <==
2& 5.38e-04 & 4.00e-04 & 8.07e-04 & 0.00 & 0.00 & 0.00 \\ 
5& 4.65e-05 & 2.67e-05 & 3.51e-05 & 2.67 & 2.95 & 3.42 \\ 
10& 7.88e-07 & 1.15e-06 & 8.88e-07 & 5.88 & 4.53 & 5.30 \\ 
20& 2.33e-08 & 2.28e-08 & 2.29e-08 & 5.08 & 5.66 & 5.28 \\ 
40& 3.85e-09 & 1.23e-09 & 2.71e-09 & 2.60 & 4.21 & 3.08 

==> figures/LinAc2D_moving_source/errors_OSS_ord2.tex <==
10& 2.34e-04 & 2.23e-04 & 9.49e-04 & 0.00 & 0.00 & 0.00 \\ 
20& 1.40e-04 & 1.40e-04 & 2.44e-04 & 0.74 & 0.67 & 1.96 \\ 
40& 4.29e-05 & 4.29e-05 & 5.26e-05 & 1.71 & 1.71 & 2.22 \\ 
80& 1.10e-05 & 1.10e-05 & 1.27e-05 & 1.97 & 1.97 & 2.05 \\ 
160& 2.75e-06 & 2.75e-06 & 3.14e-06 & 1.99 & 1.99 & 2.01 

==> figures/LinAc2D_moving_source/errors_OSS_ord3.tex <==
5& 2.65e-04 & 2.74e-04 & 7.67e-04 & 0.00 & 0.00 & 0.00 \\ 
10& 2.14e-04 & 1.21e-04 & 1.54e-04 & 0.31 & 1.17 & 2.31 \\ 
20& 4.34e-05 & 4.34e-05 & 3.43e-05 & 2.30 & 1.49 & 2.17 \\ 
40& 9.49e-06 & 9.49e-06 & 7.24e-06 & 2.19 & 2.19 & 2.25 \\ 
80& 1.96e-06 & 1.96e-06 & 1.70e-06 & 2.28 & 2.28 & 2.09 

==> figures/LinAc2D_moving_source/errors_OSS_ord4.tex <==
3& 2.86e-04 & 3.72e-04 & 8.45e-04 & 0.00 & 0.00 & 0.00 \\ 
6& 1.89e-04 & 2.06e-04 & 2.52e-04 & 0.60 & 0.85 & 1.75 \\ 
13& 1.02e-05 & 9.95e-06 & 1.98e-05 & 3.78 & 3.92 & 3.29 \\ 
26& 7.70e-07 & 7.70e-07 & 6.46e-07 & 3.73 & 3.69 & 4.94 \\ 
53& 4.36e-08 & 4.34e-08 & 2.45e-08 & 4.03 & 4.04 & 4.59 

==> figures/LinAc2D_moving_source/errors_OSS_ord5.tex <==
2& 6.69e-04 & 5.11e-04 & 1.04e-03 & 0.00 & 0.00 & 0.00 \\ 
5& 6.85e-05 & 6.44e-05 & 1.19e-04 & 2.49 & 2.26 & 2.37 \\ 
10& 5.24e-06 & 2.84e-06 & 4.25e-06 & 3.71 & 4.50 & 4.81 \\ 
20& 1.52e-07 & 1.52e-07 & 1.91e-07 & 5.11 & 4.23 & 4.48 \\ 
40& 6.04e-09 & 4.72e-09 & 9.04e-09 & 4.65 & 5.01 & 4.40 

==> figures/LinAc2D_moving_source/errors_SUPG_GF_ord2.tex <==
10& 8.01e-05 & 8.77e-05 & 1.57e-04 & 0.00 & 0.00 & 0.00 \\ 
20& 5.48e-05 & 5.48e-05 & 8.69e-05 & 0.55 & 0.68 & 0.85 \\ 
40& 1.96e-05 & 1.96e-05 & 2.36e-05 & 1.49 & 1.49 & 1.88 \\ 
80& 5.22e-06 & 5.22e-06 & 5.93e-06 & 1.91 & 1.91 & 1.99 \\ 
160& 1.32e-06 & 1.32e-06 & 1.49e-06 & 1.98 & 1.98 & 1.99 

==> figures/LinAc2D_moving_source/errors_SUPG_GF_ord3.tex <==
5& 2.44e-04 & 1.43e-04 & 4.94e-04 & 0.00 & 0.00 & 0.00 \\ 
10& 4.01e-05 & 7.02e-05 & 6.91e-05 & 2.60 & 1.03 & 2.84 \\ 
20& 5.25e-06 & 5.25e-06 & 5.98e-06 & 2.93 & 3.74 & 3.53 \\ 
40& 6.81e-07 & 6.81e-07 & 7.35e-07 & 2.95 & 2.95 & 3.02 \\ 
80& 1.13e-07 & 1.13e-07 & 8.31e-08 & 2.59 & 2.59 & 3.14 

==> figures/LinAc2D_moving_source/errors_SUPG_GF_ord4.tex <==
3& 2.76e-04 & 3.38e-04 & 6.36e-04 & 0.00 & 0.00 & 0.00 \\ 
6& 6.89e-05 & 8.63e-05 & 6.79e-05 & 2.00 & 1.97 & 3.23 \\ 
13& 2.67e-06 & 2.46e-06 & 1.90e-06 & 4.21 & 4.60 & 4.62 \\ 
26& 9.27e-08 & 9.25e-08 & 1.06e-07 & 4.85 & 4.73 & 4.17 \\ 
53& 5.60e-09 & 3.99e-09 & 6.53e-09 & 3.94 & 4.42 & 3.91 

==> figures/LinAc2D_moving_source/errors_SUPG_GF_ord5.tex <==
2& 5.71e-04 & 4.18e-04 & 7.77e-04 & 0.00 & 0.00 & 0.00 \\ 
5& 4.67e-05 & 2.61e-05 & 3.38e-05 & 2.73 & 3.03 & 3.42 \\ 
10& 7.49e-07 & 1.15e-06 & 7.38e-07 & 5.96 & 4.50 & 5.52 \\ 
20& 2.18e-08 & 2.12e-08 & 1.82e-08 & 5.10 & 5.77 & 5.34 \\ 
40& 3.93e-09 & 1.17e-09 & 2.72e-09 & 2.47 & 4.18 & 2.75 

==> figures/LinAc2D_moving_source/errors_SUPG_ord2.tex <==
10& 2.14e-04 & 1.86e-04 & 9.13e-04 & 0.00 & 0.00 & 0.00 \\ 
20& 1.27e-04 & 1.27e-04 & 2.50e-04 & 0.75 & 0.55 & 1.87 \\ 
40& 4.15e-05 & 4.15e-05 & 5.42e-05 & 1.62 & 1.62 & 2.20 \\ 
80& 1.08e-05 & 1.08e-05 & 1.29e-05 & 1.94 & 1.94 & 2.07 \\ 
160& 2.74e-06 & 2.74e-06 & 3.17e-06 & 1.98 & 1.98 & 2.02 

==> figures/LinAc2D_moving_source/errors_SUPG_ord3.tex <==
5& 2.71e-04 & 2.02e-04 & 6.96e-04 & 0.00 & 0.00 & 0.00 \\ 
10& 1.81e-04 & 1.13e-04 & 1.60e-04 & 0.59 & 0.84 & 2.12 \\ 
20& 3.09e-05 & 3.09e-05 & 2.85e-05 & 2.55 & 1.87 & 2.49 \\ 
40& 5.08e-06 & 5.08e-06 & 6.68e-06 & 2.60 & 2.60 & 2.09 \\ 
80& 7.14e-07 & 7.14e-07 & 1.33e-06 & 2.83 & 2.83 & 2.33 

==> figures/LinAc2D_moving_source/errors_SUPG_ord4.tex <==
3& 2.90e-04 & 3.90e-04 & 8.02e-04 & 0.00 & 0.00 & 0.00 \\ 
6& 1.73e-04 & 1.92e-04 & 2.23e-04 & 0.74 & 1.02 & 1.85 \\ 
13& 9.54e-06 & 8.81e-06 & 1.67e-05 & 3.75 & 3.98 & 3.35 \\ 
26& 6.61e-07 & 6.61e-07 & 6.00e-07 & 3.85 & 3.74 & 4.80 \\ 
53& 3.82e-08 & 3.79e-08 & 2.45e-08 & 4.00 & 4.01 & 4.49 

==> figures/LinAc2D_moving_source/errors_SUPG_ord5.tex <==
2& 6.73e-04 & 4.76e-04 & 9.83e-04 & 0.00 & 0.00 & 0.00 \\ 
5& 7.33e-05 & 5.49e-05 & 9.92e-05 & 2.42 & 2.36 & 2.50 \\ 
10& 3.77e-06 & 2.59e-06 & 3.49e-06 & 4.28 & 4.40 & 4.83 \\ 
20& 1.24e-07 & 1.24e-07 & 1.48e-07 & 4.92 & 4.38 & 4.56 \\ 
40& 5.93e-09 & 4.52e-09 & 7.23e-09 & 4.39 & 4.78 & 4.35 

==> figures/LinAc2D_source_vortex_dirichlet/big_table_ord2.tex <==
20 & 5.0e-03 & 2.3e-03 & 0.0 & 0.0 & 1.9e-03 & 9.5e-04 & 0.0 & 0.0 & 4.2e-03 & 3.2e-03 & 0.0 & 0.0 & 2.1e-03 & 1.3e-03 & 0.0 & 0.0 \\
40 & 1.3e-03 & 5.5e-04 & 1.9 & 2.1 & 4.1e-04 & 2.5e-04 & 2.2 & 1.9 & 9.6e-04 & 6.9e-04 & 2.1 & 2.2 & 4.5e-04 & 3.1e-04 & 2.2 & 2.0 \\
80 & 2.8e-04 & 1.3e-04 & 2.2 & 2.1 & 9.9e-05 & 6.3e-05 & 2.1 & 2.0 & 2.1e-04 & 1.5e-04 & 2.2 & 2.2 & 1.0e-04 & 7.2e-05 & 2.1 & 2.1 \\
160 & 5.8e-05 & 3.2e-05 & 2.3 & 2.0 & 2.5e-05 & 1.6e-05 & 2.0 & 2.0 & 5.1e-05 & 3.4e-05 & 2.1 & 2.1 & 2.5e-05 & 1.7e-05 & 2.0 & 2.1 \\
320 & 1.3e-05 & 7.7e-06 & 2.2 & 2.0 & 6.2e-06 & 3.8e-06 & 2.0 & 2.0 & 1.2e-05 & 8.1e-06 & 2.0 & 2.1 & 6.2e-06 & 4.0e-06 & 2.0 & 2.1 

==> figures/LinAc2D_source_vortex_dirichlet/big_table_ord3.tex <==
10 & 4.9e-03 & 1.5e-03 & 0.0 & 0.0 & 1.9e-03 & 9.0e-04 & 0.0 & 0.0 & 4.3e-03 & 2.5e-03 & 0.0 & 0.0 & 2.1e-03 & 1.4e-03 & 0.0 & 0.0 \\
20 & 1.6e-03 & 3.1e-04 & 1.6 & 2.3 & 2.2e-04 & 8.6e-05 & 3.2 & 3.4 & 1.1e-03 & 4.4e-04 & 2.0 & 2.5 & 2.4e-04 & 1.4e-04 & 3.1 & 3.4 \\
40 & 4.4e-04 & 7.4e-05 & 1.8 & 2.1 & 1.8e-05 & 6.1e-06 & 3.6 & 3.8 & 3.0e-04 & 7.1e-05 & 1.8 & 2.6 & 1.9e-05 & 9.1e-06 & 3.7 & 3.9 \\
80 & 1.1e-04 & 1.7e-05 & 2.0 & 2.2 & 1.2e-06 & 4.6e-07 & 3.9 & 3.7 & 9.2e-05 & 1.7e-05 & 1.7 & 2.1 & 1.2e-06 & 5.3e-07 & 4.0 & 4.1 \\
160 & 2.4e-05 & 3.1e-06 & 2.2 & 2.4 & 7.2e-08 & 3.3e-08 & 4.0 & 3.8 & 2.6e-05 & 4.7e-06 & 1.8 & 1.8 & 7.4e-08 & 3.4e-08 & 4.0 & 4.0 

==> figures/LinAc2D_source_vortex_dirichlet/big_table_ord4.tex <==
6 & 5.5e-03 & 1.7e-03 & 0.0 & 0.0 & 1.8e-03 & 6.4e-04 & 0.0 & 0.0 & 5.4e-03 & 2.0e-03 & 0.0 & 0.0 & 1.8e-03 & 7.0e-04 & 0.0 & 0.0 \\
13 & 1.1e-03 & 2.0e-04 & 2.0 & 2.8 & 1.9e-04 & 6.1e-05 & 2.9 & 3.0 & 1.1e-03 & 2.4e-04 & 2.0 & 2.7 & 1.9e-04 & 6.5e-05 & 2.9 & 3.1 \\
26 & 1.8e-04 & 1.5e-05 & 2.6 & 3.8 & 1.1e-05 & 3.5e-06 & 4.1 & 4.1 & 1.8e-04 & 1.7e-05 & 2.6 & 3.8 & 1.1e-05 & 3.7e-06 & 4.1 & 4.2 \\
53 & 1.7e-05 & 1.1e-06 & 3.4 & 3.7 & 4.1e-07 & 1.1e-07 & 4.7 & 4.9 & 1.6e-05 & 1.2e-06 & 3.4 & 3.8 & 4.1e-07 & 1.1e-07 & 4.7 & 4.9 \\
106 & 1.3e-06 & 6.7e-08 & 3.7 & 4.0 & 1.3e-08 & 1.9e-09 & 4.9 & 5.9 & 1.2e-06 & 6.8e-08 & 3.8 & 4.1 & 1.4e-08 & 3.2e-09 & 4.9 & 5.2 

==> figures/LinAc2D_source_vortex_dirichlet/big_table_ord5.tex <==
5 & 4.2e-03 & 1.0e-03 & 0.0 & 0.0 & 1.6e-03 & 5.8e-04 & 0.0 & 0.0 & 4.0e-03 & 1.3e-03 & 0.0 & 0.0 & 1.6e-03 & 6.7e-04 & 0.0 & 0.0 \\
10 & 8.8e-04 & 9.1e-05 & 2.2 & 3.5 & 1.9e-04 & 5.3e-05 & 3.1 & 3.5 & 8.8e-04 & 1.1e-04 & 2.2 & 3.6 & 2.0e-04 & 5.8e-05 & 3.1 & 3.5 \\
20 & 8.9e-05 & 6.9e-06 & 3.3 & 3.7 & 7.6e-06 & 1.8e-06 & 4.7 & 4.9 & 8.8e-05 & 8.7e-06 & 3.3 & 3.6 & 7.6e-06 & 1.9e-06 & 4.7 & 4.9 \\
40 & 5.5e-06 & 2.7e-07 & 4.0 & 4.7 & 1.9e-07 & 3.8e-08 & 5.4 & 5.6 & 5.4e-06 & 3.4e-07 & 4.0 & 4.7 & 1.9e-07 & 3.9e-08 & 5.4 & 5.6 \\
80 & 3.3e-07 & 1.5e-08 & 4.0 & 4.2 & 3.3e-09 & 6.7e-10 & 5.8 & 5.8 & 3.3e-07 & 2.0e-08 & 4.0 & 4.1 & 5.4e-09 & 3.1e-09 & 5.1 & 3.7 

==> figures/LinAc2D_source_vortex_dirichlet/big_table_ord6.tex <==
4 & 4.0e-03 & 1.1e-03 & 0.0 & 0.0 & 2.0e-03 & 8.2e-04 & 0.0 & 0.0 & 3.9e-03 & 1.4e-03 & 0.0 & 0.0 & 2.0e-03 & 9.5e-04 & 0.0 & 0.0 \\
8 & 6.6e-04 & 5.7e-05 & 2.6 & 4.3 & 1.5e-04 & 3.2e-05 & 3.8 & 4.7 & 6.4e-04 & 7.5e-05 & 2.6 & 4.2 & 1.5e-04 & 3.6e-05 & 3.8 & 4.7 \\
16 & 5.3e-05 & 2.8e-06 & 3.6 & 4.3 & 6.2e-06 & 1.3e-06 & 4.5 & 4.6 & 5.3e-05 & 3.9e-06 & 3.6 & 4.3 & 6.2e-06 & 1.4e-06 & 4.5 & 4.7 \\
32 & 2.9e-06 & 1.2e-07 & 4.2 & 4.5 & 1.1e-07 & 2.2e-08 & 5.8 & 5.9 & 2.7e-06 & 1.8e-07 & 4.3 & 4.4 & 1.1e-07 & 2.3e-08 & 5.8 & 5.9 \\
64 & 8.5e-08 & 2.5e-09 & 5.1 & 5.6 & 1.1e-09 & 1.1e-10 & 6.6 & 7.6 & 8.0e-08 & 5.3e-09 & 5.1 & 5.1 & 5.1e-09 & 3.4e-09 & 4.4 & 2.8 

==> figures/LinAc2D_source_vortex_dirichlet/errors_OSS_GF_ord2.tex <==
20& 2.10e-03 & 2.15e-03 & 1.27e-03 & 0.00 & 0.00 & 0.00 \\ 
40& 4.48e-04 & 4.64e-04 & 3.14e-04 & 2.23 & 2.21 & 2.02 \\ 
80& 1.03e-04 & 1.08e-04 & 7.22e-05 & 2.12 & 2.11 & 2.12 \\ 
160& 2.52e-05 & 2.63e-05 & 1.68e-05 & 2.03 & 2.03 & 2.10 \\ 
320& 6.23e-06 & 6.50e-06 & 4.00e-06 & 2.02 & 2.02 & 2.07 

==> figures/LinAc2D_source_vortex_dirichlet/errors_OSS_GF_ord3.tex <==
10& 2.09e-03 & 2.21e-03 & 1.42e-03 & 0.00 & 0.00 & 0.00 \\ 
20& 2.41e-04 & 2.40e-04 & 1.37e-04 & 3.11 & 3.20 & 3.38 \\ 
40& 1.87e-05 & 1.87e-05 & 9.08e-06 & 3.69 & 3.68 & 3.91 \\ 
80& 1.19e-06 & 1.19e-06 & 5.31e-07 & 3.98 & 3.98 & 4.10 \\ 
160& 7.44e-08 & 7.43e-08 & 3.35e-08 & 4.00 & 4.00 & 3.98 

==> figures/LinAc2D_source_vortex_dirichlet/errors_OSS_GF_ord4.tex <==
6& 1.78e-03 & 1.69e-03 & 7.00e-04 & 0.00 & 0.00 & 0.00 \\ 
13& 1.91e-04 & 1.89e-04 & 6.51e-05 & 2.88 & 2.83 & 3.07 \\ 
26& 1.14e-05 & 1.14e-05 & 3.66e-06 & 4.07 & 4.06 & 4.15 \\ 
53& 4.08e-07 & 4.08e-07 & 1.14e-07 & 4.67 & 4.67 & 4.86 \\ 
106& 1.39e-08 & 1.41e-08 & 3.20e-09 & 4.88 & 4.85 & 5.16 

==> figures/LinAc2D_source_vortex_dirichlet/errors_OSS_GF_ord5.tex <==
5& 1.62e-03 & 1.58e-03 & 6.68e-04 & 0.00 & 0.00 & 0.00 \\ 
10& 1.96e-04 & 1.96e-04 & 5.82e-05 & 3.05 & 3.01 & 3.52 \\ 
20& 7.60e-06 & 7.60e-06 & 1.92e-06 & 4.69 & 4.69 & 4.92 \\ 
40& 1.86e-07 & 1.86e-07 & 3.90e-08 & 5.35 & 5.35 & 5.62 \\ 
80& 5.43e-09 & 6.01e-09 & 3.08e-09 & 5.10 & 4.95 & 3.66 

==> figures/LinAc2D_source_vortex_dirichlet/errors_OSS_GF_ord6.tex <==
4& 2.44e-03 & 2.83e-03 & 1.01e-03 & 0.00 & 0.00 & 0.00 \\ 
8& 1.55e-04 & 1.56e-04 & 3.92e-05 & 3.98 & 4.18 & 4.69 \\ 
16& 6.27e-06 & 6.27e-06 & 1.38e-06 & 4.62 & 4.64 & 4.82 \\ 
32& 1.11e-07 & 1.11e-07 & 2.36e-08 & 5.82 & 5.81 & 5.87 \\ 
64& 5.12e-09 & 5.30e-09 & 3.41e-09 & 4.44 & 4.39 & 2.79 

==> figures/LinAc2D_source_vortex_dirichlet/errors_OSS_GF_ord7.tex <==
3& 4.55e-03 & 4.00e-03 & 1.60e-03 & 0.00 & 0.00 & 0.00 \\ 
6& 6.33e-04 & 7.51e-04 & 4.11e-04 & 2.85 & 2.41 & 1.97 \\ 
13& 6.86e-04 & 6.85e-04 & 4.03e-04 & -0.10 & 0.12 & 0.02 \\ 
26& 6.91e-04 & 6.91e-04 & 4.04e-04 & -0.01 & -0.01 & -0.00 \\ 
53& 6.93e-04 & 6.93e-04 & 4.05e-04 & -0.00 & -0.00 & -0.00 

==> figures/LinAc2D_source_vortex_dirichlet/errors_OSS_ord2.tex <==
20& 4.20e-03 & 4.32e-03 & 3.21e-03 & 0.00 & 0.00 & 0.00 \\ 
40& 9.57e-04 & 9.88e-04 & 6.95e-04 & 2.13 & 2.13 & 2.21 \\ 
80& 2.12e-04 & 2.20e-04 & 1.48e-04 & 2.18 & 2.17 & 2.23 \\ 
160& 5.05e-05 & 5.27e-05 & 3.39e-05 & 2.07 & 2.06 & 2.13 \\ 
320& 1.24e-05 & 1.30e-05 & 8.05e-06 & 2.02 & 2.02 & 2.07 

==> figures/LinAc2D_source_vortex_dirichlet/errors_OSS_ord3.tex <==
10& 4.32e-03 & 4.04e-03 & 2.52e-03 & 0.00 & 0.00 & 0.00 \\ 
20& 1.07e-03 & 1.07e-03 & 4.37e-04 & 2.01 & 1.92 & 2.53 \\ 
40& 3.04e-04 & 2.97e-04 & 7.08e-05 & 1.81 & 1.85 & 2.62 \\ 
80& 9.17e-05 & 8.81e-05 & 1.66e-05 & 1.73 & 1.75 & 2.10 \\ 
160& 2.63e-05 & 2.53e-05 & 4.70e-06 & 1.80 & 1.80 & 1.82 

==> figures/LinAc2D_source_vortex_dirichlet/errors_OSS_ord4.tex <==
6& 5.41e-03 & 5.38e-03 & 1.97e-03 & 0.00 & 0.00 & 0.00 \\ 
13& 1.12e-03 & 1.07e-03 & 2.38e-04 & 2.03 & 2.09 & 2.73 \\ 
26& 1.83e-04 & 1.84e-04 & 1.70e-05 & 2.61 & 2.54 & 3.81 \\ 
53& 1.65e-05 & 1.65e-05 & 1.16e-06 & 3.38 & 3.39 & 3.76 \\ 
106& 1.21e-06 & 1.21e-06 & 6.84e-08 & 3.77 & 3.77 & 4.09 

==> figures/LinAc2D_source_vortex_dirichlet/errors_OSS_ord5.tex <==
5& 4.02e-03 & 3.40e-03 & 1.31e-03 & 0.00 & 0.00 & 0.00 \\ 
10& 8.76e-04 & 8.85e-04 & 1.09e-04 & 2.20 & 1.94 & 3.59 \\ 
20& 8.77e-05 & 8.78e-05 & 8.74e-06 & 3.32 & 3.33 & 3.65 \\ 
40& 5.43e-06 & 5.43e-06 & 3.38e-07 & 4.01 & 4.01 & 4.69 \\ 
80& 3.28e-07 & 3.28e-07 & 2.03e-08 & 4.05 & 4.05 & 4.05 

==> figures/LinAc2D_source_vortex_dirichlet/errors_OSS_ord6.tex <==
4& 3.86e-03 & 4.17e-03 & 1.36e-03 & 0.00 & 0.00 & 0.00 \\ 
8& 6.41e-04 & 6.44e-04 & 7.49e-05 & 2.59 & 2.70 & 4.18 \\ 
16& 5.28e-05 & 5.29e-05 & 3.91e-06 & 3.60 & 3.61 & 4.26 \\ 
32& 2.69e-06 & 2.69e-06 & 1.85e-07 & 4.29 & 4.29 & 4.40 \\ 
64& 7.98e-08 & 7.98e-08 & 5.35e-09 & 5.08 & 5.08 & 5.11 

==> figures/LinAc2D_source_vortex_dirichlet/errors_OSS_ord7.tex <==
3& 6.43e-03 & 6.52e-03 & 2.00e-03 & 0.00 & 0.00 & 0.00 \\ 
6& 8.91e-04 & 9.63e-04 & 4.23e-04 & 2.85 & 2.76 & 2.24 \\ 
13& 6.88e-04 & 6.86e-04 & 4.04e-04 & 0.33 & 0.44 & 0.06 \\ 
26& 6.91e-04 & 6.91e-04 & 4.04e-04 & -0.01 & -0.01 & -0.00 \\ 
53& 6.93e-04 & 6.93e-04 & 4.05e-04 & -0.00 & -0.00 & -0.00 

==> figures/LinAc2D_source_vortex_dirichlet/errors_SUPG_GF_ord2.tex <==
20& 1.86e-03 & 1.92e-03 & 9.54e-04 & 0.00 & 0.00 & 0.00 \\ 
40& 4.12e-04 & 4.29e-04 & 2.55e-04 & 2.17 & 2.16 & 1.90 \\ 
80& 9.94e-05 & 1.04e-04 & 6.32e-05 & 2.05 & 2.05 & 2.01 \\ 
160& 2.47e-05 & 2.58e-05 & 1.57e-05 & 2.01 & 2.01 & 2.01 \\ 
320& 6.17e-06 & 6.44e-06 & 3.84e-06 & 2.00 & 2.00 & 2.03 

==> figures/LinAc2D_source_vortex_dirichlet/errors_SUPG_GF_ord3.tex <==
10& 1.92e-03 & 2.02e-03 & 9.00e-04 & 0.00 & 0.00 & 0.00 \\ 
20& 2.15e-04 & 2.14e-04 & 8.55e-05 & 3.15 & 3.24 & 3.40 \\ 
40& 1.78e-05 & 1.78e-05 & 6.06e-06 & 3.59 & 3.59 & 3.82 \\ 
80& 1.16e-06 & 1.15e-06 & 4.65e-07 & 3.95 & 3.95 & 3.70 \\ 
160& 7.22e-08 & 7.20e-08 & 3.26e-08 & 4.00 & 4.00 & 3.84 

==> figures/LinAc2D_source_vortex_dirichlet/errors_SUPG_GF_ord4.tex <==
6& 1.77e-03 & 1.69e-03 & 6.40e-04 & 0.00 & 0.00 & 0.00 \\ 
13& 1.90e-04 & 1.88e-04 & 6.06e-05 & 2.88 & 2.84 & 3.05 \\ 
26& 1.13e-05 & 1.13e-05 & 3.51e-06 & 4.07 & 4.06 & 4.11 \\ 
53& 4.06e-07 & 4.06e-07 & 1.09e-07 & 4.67 & 4.67 & 4.87 \\ 
106& 1.34e-08 & 1.34e-08 & 1.88e-09 & 4.92 & 4.92 & 5.86 

==> figures/LinAc2D_source_vortex_dirichlet/errors_SUPG_GF_ord5.tex <==
5& 1.62e-03 & 1.57e-03 & 5.83e-04 & 0.00 & 0.00 & 0.00 \\ 
10& 1.95e-04 & 1.95e-04 & 5.33e-05 & 3.05 & 3.01 & 3.45 \\ 
20& 7.59e-06 & 7.59e-06 & 1.79e-06 & 4.68 & 4.68 & 4.89 \\ 
40& 1.86e-07 & 1.86e-07 & 3.77e-08 & 5.35 & 5.35 & 5.57 \\ 
80& 3.29e-09 & 3.29e-09 & 6.73e-10 & 5.82 & 5.82 & 5.81 

==> figures/LinAc2D_source_vortex_dirichlet/errors_SUPG_GF_ord6.tex <==
4& 2.00e-03 & 2.00e-03 & 8.19e-04 & 0.00 & 0.00 & 0.00 \\ 
8& 1.46e-04 & 1.46e-04 & 3.19e-05 & 3.78 & 3.78 & 4.68 \\ 
16& 6.24e-06 & 6.24e-06 & 1.29e-06 & 4.55 & 4.55 & 4.63 \\ 
32& 1.08e-07 & 1.08e-07 & 2.17e-08 & 5.85 & 5.85 & 5.89 \\ 
64& 1.11e-09 & 1.11e-09 & 1.13e-10 & 6.61 & 6.61 & 7.59 

==> figures/LinAc2D_source_vortex_dirichlet/errors_SUPG_GF_ord7.tex <==
3& 3.62e-03 & 3.57e-03 & 1.37e-03 & 0.00 & 0.00 & 0.00 \\ 
6& 1.54e-04 & 1.54e-04 & 5.80e-05 & 4.55 & 4.53 & 4.56 \\ 
13& 7.14e-06 & 7.14e-06 & 2.16e-06 & 3.97 & 3.98 & 4.25 \\ 
26& 9.16e-08 & 9.16e-08 & 1.65e-08 & 6.29 & 6.29 & 7.03 \\ 
53& 4.81e-10 & 4.81e-10 & 7.65e-11 & 7.37 & 7.37 & 7.55 

==> figures/LinAc2D_source_vortex_dirichlet/errors_SUPG_ord2.tex <==
20& 4.96e-03 & 5.07e-03 & 2.33e-03 & 0.00 & 0.00 & 0.00 \\ 
40& 1.30e-03 & 1.32e-03 & 5.52e-04 & 1.94 & 1.94 & 2.08 \\ 
80& 2.80e-04 & 2.86e-04 & 1.30e-04 & 2.21 & 2.20 & 2.09 \\ 
160& 5.84e-05 & 6.02e-05 & 3.15e-05 & 2.26 & 2.25 & 2.04 \\ 
320& 1.30e-05 & 1.35e-05 & 7.71e-06 & 2.16 & 2.15 & 2.03 

==> figures/LinAc2D_source_vortex_dirichlet/errors_SUPG_ord3.tex <==
10& 4.86e-03 & 4.85e-03 & 1.55e-03 & 0.00 & 0.00 & 0.00 \\ 
20& 1.56e-03 & 1.49e-03 & 3.11e-04 & 1.64 & 1.70 & 2.32 \\ 
40& 4.39e-04 & 4.24e-04 & 7.43e-05 & 1.83 & 1.81 & 2.06 \\ 
80& 1.09e-04 & 1.07e-04 & 1.66e-05 & 2.01 & 1.98 & 2.16 \\ 
160& 2.39e-05 & 2.39e-05 & 3.06e-06 & 2.19 & 2.17 & 2.44 

==> figures/LinAc2D_source_vortex_dirichlet/errors_SUPG_ord4.tex <==
6& 5.45e-03 & 5.37e-03 & 1.71e-03 & 0.00 & 0.00 & 0.00 \\ 
13& 1.13e-03 & 1.08e-03 & 2.03e-04 & 2.03 & 2.08 & 2.76 \\ 
26& 1.84e-04 & 1.85e-04 & 1.50e-05 & 2.62 & 2.54 & 3.76 \\ 
53& 1.69e-05 & 1.70e-05 & 1.06e-06 & 3.35 & 3.36 & 3.71 \\ 
106& 1.29e-06 & 1.29e-06 & 6.72e-08 & 3.71 & 3.71 & 3.98 

==> figures/LinAc2D_source_vortex_dirichlet/errors_SUPG_ord5.tex <==
5& 4.17e-03 & 3.52e-03 & 1.04e-03 & 0.00 & 0.00 & 0.00 \\ 
10& 8.80e-04 & 8.90e-04 & 9.08e-05 & 2.25 & 1.98 & 3.52 \\ 
20& 8.88e-05 & 8.89e-05 & 6.86e-06 & 3.31 & 3.32 & 3.73 \\ 
40& 5.47e-06 & 5.48e-06 & 2.66e-07 & 4.02 & 4.02 & 4.69 \\ 
80& 3.35e-07 & 3.35e-07 & 1.50e-08 & 4.03 & 4.03 & 4.15 

==> figures/LinAc2D_source_vortex_dirichlet/errors_SUPG_ord6.tex <==
4& 4.01e-03 & 4.37e-03 & 1.09e-03 & 0.00 & 0.00 & 0.00 \\ 
8& 6.55e-04 & 6.60e-04 & 5.69e-05 & 2.61 & 2.73 & 4.26 \\ 
16& 5.35e-05 & 5.35e-05 & 2.81e-06 & 3.62 & 3.62 & 4.34 \\ 
32& 2.87e-06 & 2.87e-06 & 1.22e-07 & 4.22 & 4.22 & 4.53 \\ 
64& 8.52e-08 & 8.52e-08 & 2.48e-09 & 5.08 & 5.08 & 5.62 

==> figures/LinAc2D_source_vortex_dirichlet/errors_SUPG_ord7.tex <==
3& 6.44e-03 & 6.49e-03 & 1.81e-03 & 0.00 & 0.00 & 0.00 \\ 
6& 6.24e-04 & 6.24e-04 & 1.05e-04 & 3.37 & 3.38 & 4.11 \\ 
13& 5.02e-05 & 5.02e-05 & 3.71e-06 & 3.26 & 3.26 & 4.32 \\ 
26& 1.63e-06 & 1.63e-06 & 5.81e-08 & 4.94 & 4.94 & 6.00 \\ 
53& 2.32e-08 & 2.32e-08 & 9.68e-10 & 5.98 & 5.98 & 5.75 

==> tikz-OSS-coriolis.tex <==
\begin{figure} 
	\centering
		\begin{tikzpicture}
			\begin{axis}[
				xmode=log, ymode=log,
				xmin=2.6,xmax=1000,
				%ymin=1.e-9,ymax=1.,
				grid=major,
				xlabel={$N$},
				ylabel={$L^2$ Error of $u$},
				xlabel shift = 1 pt,
				ylabel shift = 1 pt,
				legend pos= north east,
				legend style={nodes={scale=0.6, transform shape}},
				width=.95\textwidth,
				height=.4\textwidth
				]
				
				\addplot[mark=square*,mark size=1.3pt,densely dashdotted, magenta]             table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_ord2.csv};
				\addlegendentry{OSS2}
				\addplot[mark=square*,dashed,mark size=1.3pt,magenta]  table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord2.csv};
				\addlegendentry{OSS-GFq2}
				\addplot[magenta,domain=20:320]{500./x/x};
				\addlegendentry{order 2}		
				
				\addplot[mark=otimes*,mark size=1.3pt,densely dashdotted, blue]             table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_ord3.csv};
				\addlegendentry{OSS3}
				\addplot[mark=otimes*,dashed,mark size=1.3pt,blue]  table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord3.csv};
				\addlegendentry{OSS-GFq3}
				\addplot[blue,domain=10:160]{500./x/x/x};
				\addlegendentry{order 3}		
				
				\addplot[mark=triangle*,mark size=1.3pt,densely dashdotted, violet]             table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_ord4.csv};
				\addlegendentry{OSS4}
				\addplot[mark=triangle*,dashed,mark size=1.3pt,violet]  table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord4.csv};
				\addlegendentry{OSS-GFq4}
				\addplot[violet,domain=6:106]{500./x/x/x/x};
				\addlegendentry{order 4}			
				
				\addplot[mark=star,mark size=1.3pt,densely dashdotted, red]             table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_ord5.csv};
				\addlegendentry{OSS5}
				\addplot[mark=star,dashed,mark size=1.3pt,red]  table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord51.csv};
				\addlegendentry{OSS-GFq5}
				\addplot[red,domain=5:80]{500./x/x/x/x/x};
				\addlegendentry{order 5}	
				
				\addplot[mark=diamond*,mark size=1.3pt,densely dashdotted,olive]             table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_ord61.csv};
				\addlegendentry{OSS6}
				\addplot[mark=diamond*,dashed,mark size=1.3pt,olive]  table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord61.csv};
				\addlegendentry{OSS-GFq6}
				\addplot[olive,domain=4:64]{500./x/x/x/x/x/x};
				\addlegendentry{order 6}				
			\end{axis}
	\end{tikzpicture}
	\caption{Steady vortex with Coriolis force: convergence of $L^2$ error in $u$ w.r.t. the number of elements in $x$ for the OSS stabilized schemes.}\label{fig:convergence_vort_coriolis-OSS}
\end{figure}



==> tikz-SU-coriolis.tex <==
\begin{figure} 
	\centering
		\begin{tikzpicture}
			\begin{axis}[
				xmode=log, ymode=log,
				xmin=2.6,xmax=1000,
				%ymin=1.e-9,ymax=1.,
				grid=major,
				xlabel={$N$},
				ylabel={$L^2$ Error of $u$},
				xlabel shift = 1 pt,
				ylabel shift = 1 pt,
				legend pos= north east,
				legend style={nodes={scale=0.6, transform shape}},
				width=.95\textwidth,
				height=.4\textwidth
				]
				
				\addplot[mark=square*,mark size=1.3pt,densely dashdotted, magenta]             table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_ord2.csv};
				\addlegendentry{SU2}
				\addplot[mark=square*,dashed,mark size=1.3pt,magenta]  table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord2.csv};
				\addlegendentry{SU-GFq2}
				\addplot[magenta,domain=20:320]{500./x/x};
				\addlegendentry{order 2}		
				
				\addplot[mark=otimes*,mark size=1.3pt,densely dashdotted, blue]             table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_ord3.csv};
				\addlegendentry{SU3}
				\addplot[mark=otimes*,dashed,mark size=1.3pt,blue]  table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord3.csv};
				\addlegendentry{SU-GFq3}
				\addplot[blue,domain=10:160]{500./x/x/x};
				\addlegendentry{order 3}		
				
				\addplot[mark=triangle*,mark size=1.3pt,densely dashdotted, violet]             table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_ord4.csv};
				\addlegendentry{SU4}
				\addplot[mark=triangle*,dashed,mark size=1.3pt,violet]  table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord4.csv};
				\addlegendentry{SU-GFq4}
				\addplot[violet,domain=6:106]{500./x/x/x/x};
				\addlegendentry{order 4}			
				
				\addplot[mark=star,mark size=1.3pt,densely dashdotted, red]             table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_ord5.csv};
				\addlegendentry{SU5}
				\addplot[mark=star,dashed,mark size=1.3pt,red]  table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord51.csv};
				\addlegendentry{SU-GFq5}
				\addplot[red,domain=5:80]{500./x/x/x/x/x};
				\addlegendentry{order 5}	
				
				\addplot[mark=diamond*,mark size=1.3pt,densely dashdotted,olive]             table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_ord61.csv};
				\addlegendentry{SU6}
				\addplot[mark=diamond*,dashed,mark size=1.3pt,olive]  table [y=err u, x=N, col sep=comma]{figures/LinAc2D_coriolis_vortex/errors_OSS_GF_ord61.csv};
				\addlegendentry{SU-GFq6}
				\addplot[olive,domain=4:64]{500./x/x/x/x/x/x};
				\addlegendentry{order 6}				
			\end{axis}
	\end{tikzpicture}
	\caption{Steady vortex with Coriolis force: convergence of $L^2$ error in $u$ w.r.t. the number of elements in $x$ for the SU stabilized schemes.}\label{fig:convergence_vort_coriolis-SUPG}
\end{figure}
